Community Detection in Networks with Node Features

Many methods have been proposed for community detection in networks, but most of them do not take into account additional information on the nodes that is often available in practice. In this paper, we propose a new joint community detection criterion that uses both the network edge information and the node features to detect community structures. One advantage our method has over existing joint detection approaches is the flexibility of learning the impact of different features which may differ across communities. Another advantage is the flexibility of choosing the amount of influence the feature information has on communities. The method is asymptotically consistent under the block model with additional assumptions on the feature distributions, and performs well on simulated and real networks.

==> texsections/commented_out.tex <==
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      SECTION 2
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \section{Notations and preliminaries}
% We first introduce notation that we are going to use for the rest of this paper. We denote the adjacency matrix for the observed networkf $A$, where $A_{ij}=1$ if nodes $i$ and $j$ are connected. Throughout this paper we consider undirected networks, i.e., $A_{ij}=A_{ji}$. On each node, there is a node feature vector, each element representing one aspect of the node's profile. For example, in a school friendship network, a student's feature vector might be $(f, 10, (0,1,0,1))$, where $f$ represents gender, $10$ is her grade and the binary vector $(0,1,0,1)$ describes her interests in four school sports activities("football", "soccer", "basketball" and "baseball").\\
% 
% Next, we define the concept of communities which we are targeting. We assume there exists an underlying partition $C:=(C_1, \ldots, C_K)$ of all nodes into $K$ communities. Nodes within the same community tend to more intensively connect to each other and have higher similarities in their features. I.e., if we have a similarity measure $\phi$, then:
% \begin{align}
% \mathbb{P}(A_{ij}=1|(i, j)\in C_k) &> \mathbb{P}(A_{ij}=1)\\
% \mathbb{E}[\phi_{ij}|(i, j)\in C_k] &> \mathbb{E}[\phi_{ij}]
% \end{align}
% We do not specify the dependence between $A$ and $F$ marginally or given $C$ since our approach is not based on a specific generative model. However, in the simulation studies later we generate conditionally independent $A$ and $F$ given $C$. Throughout this paper, we always assume that the clustering structures present in $A$ and $F$ are consistent. If the information from one of them is irrelevant to the target community structure, the joint method is expected to be inferior to the marginal method making use of the relevant source. It is natural to expect that introducing additional and potentially misleading information will do harm to the estimation outcome, whatever method is used.








% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      SECTION 8
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Future work}
% 
% A major aspect of future work is to explore the extendability of our method to the overlapping communities case. Notice that the JCDC is decomposed into summands along each community, i.e., the joint community detection criterion can be written as:
% \begin{equation}
% 	R = \sum_{k=1}^K T(C_k, A, \bm{w})
% \end{equation}
% where $T$ is the rescaled sum of weighted edges in community $k$. The issue emerges that the global optimum is achieved by assigning each community the same set of members that maximizes the individual summand. We are interested in remedying this issue and assessing the performance of the detection criterion under the overlapping communities scenario.\\
% 
% Also, the current criterion does not consider degree correction on the network $A$. In some networks, node degrees may be related to their features. For example, from a generative point of view, nodes at central positions in the feature space tend to have high similarity to many other nodes and therefore connect to many other nodes while for similar reasons peripheral nodes have lower degrees. Otherwise, in contexts where node features and degrees are independent, we are interested in taking the degree correction into consideration to refine the available community structure on the network.

==> texsections/proof__Yuan_Zhang____________2015-07-24_.tex <==
We start with defining notation. Let $\E_k$ denote the set of nodes belonging to the $k$th estimated community and ${\cal C}_k$ denote the node set of the $k$th true community. Then by definition $e=\{{\cal E}_1, \ldots, \E_k\}$ and $c=\{{\cal C}_1,\ldots, {\cal C}_K\}$. Recall the joint community detection criterion is
\begin{equation*}
	R(e, \beta; w_n) = \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} A_{ij}W(\phi_{ij}, \beta_k; w_n)
\end{equation*}
Define $R^0$, the ``population version criterion'', as follows:
\begin{equation*}
	R^0(e, \beta; w_n) := \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} \rho_n P_{c_ic_j}\mathbb{E}[W(\phi_{ij}, \beta_k; w_n)]
\end{equation*}
The expectation in $R^0$ is taken on node features.

\begin{lemma}\label{lemma_1}
Under conditions \ref{condition_1} and \ref{condition_2}, choose $w_n$ such that $w_n\rho_n\to \infty$ and $0<\alpha<1$, we have
\begin{align*}
  \max_{e,\beta} \frac{\left| R(e, \beta; w_n) - R^0(e, \beta; w_n) \right|}{w_n \rho_n n^{2-\alpha}} = O_p\left(\frac{1}{\sqrt{w_n\rho_n}}\right)
\end{align*}
\end{lemma}

\begin{proof}[of Lemma~\ref{lemma_1}]
We first bound the difference between $R$ and $R^0$ for fixed $e$ and $\beta$. By Hoeffding's inequality,
\begin{align*}
  \prb\left\{\left| \frac{1}{|\E_k|^2} \sum_{i, j\in \E_k} \left( A_{ij}\wijbkwn-\rho_nP_{c_ic_j} \ep[\wijbkwn] \right) \right| > t \right\}\leq 2\exp\left( -2[n/2] t^2/w_n^2 \right)
\end{align*}
Taking $t=w_n\rho_n n^{2-\alpha} \delta/|\E_k|^{2-\alpha}$ and by the union bound, we have:
\begin{align*}
&\prb\left( \frac{|R(e, \beta; w_n) - R^0(e, \beta; w_n)|}{w_n\rho_n n^{2-\alpha}} > K\delta \right)\\
\leq & \sum_{k=1}^K \prb \left\{ \frac{ \big| \sum_{i,j\in \E_k} \left( A_{ij}\wijbkwn - \rho_nP_{c_ic_j} \ep\left[ \wijbkwn \right] \right) \big| }{ w_n\rho_n|\E_k|^\alpha n^{2-\alpha} } \geq \delta \right\}\\
\leq & \sum_{k=1}^K 2\exp\left\{ -2[n/2] w_n^2 \rho_n^2 n^{4-2\alpha}\delta^2/|\E_k|^{4-2\alpha} \right\} \leq 2K\exp\left\{ -(n-1)w_n^2\rho_n^2\delta^2 \right\}
\end{align*}
Then we take the uniform bound over $\beta$. Consider the following set:
\begin{equation*}
B_\epsilon:=\left\{ \left(\frac{s_1 \epsilon}{ \sqrt{p}},\ldots, \frac{s_p \epsilon}{ \sqrt{p}} \right), s_1,\ldots,s_p\in\left\{ 0, \pm 1,\ldots,\pm \left[ \frac{2M_\beta\sqrt{p}}{\epsilon} \right] \right\}\cup \left\{ \pm\frac{2M_\beta\sqrt{p}}{\epsilon} \right\} \right\}
\end{equation*}
It is easy to verify that $B_\epsilon$ is an $\epsilon-$net of $[-M_\beta, M_\beta]^p$, the sample space of $\beta_k$. For each $\beta_k$, let $\beta(\beta_k, B_\epsilon)$ be the best approximation to $\beta_k$ in $B_\epsilon$, we have:
\begin{align*}
\max_{\beta_k} |\wijbkwn - W(\phi_{ij}, \beta(\beta_k, B_\epsilon); w_n)|&\leq \max_{\beta_k} \left| \frac{\partial w}{\partial \beta_k}(\phi_ij, \beta_k; w_n) \right| |\beta_k - \beta(\beta_k, B_\epsilon)|\\
&\leq M_\phi M_\beta \exp(M_\phi M_\beta) \epsilon \leq M_\phi M_\beta w_n\epsilon
\end{align*}
Therefore,
\begin{align*}
& \prb\left( \max_\beta \frac{|R(e, \beta; w_n) - R^0(e, \beta; w_n)|}{w_n\rho_n n^{2-\alpha}} > K\delta \right)\leq \sum_{k=1}^K \prb\left\{ \max_{\beta_k} \frac{\left| (A_{ij} - \rho_nP_{c_ic_j})\wijbkwn \right|}{w_n\rho_n|\E_k|^\alpha n^{2-\alpha}} >\delta \right\}\\
\leq & \sum_{k=1}^K \prb\left\{ \max_{\beta_k} \frac{ \sum_{i,j\in\E_k} |A_{ij} - \rho_nP_{c_ic_j}| |\wijbkwn - W(\phi_{ij}, \beta(\beta_k, B_\epsilon); w_n)| }{w_n\rho_n|\E_k|^\alpha n^{2-\alpha}} > \frac{\delta}{2} \right\}\\
+ & \sum_{k=1}^K \prb\left\{ \max_{\beta_0\in B_\epsilon} \frac{ \left| \sum_{i,j\in\E_k} \left(A_{ij} - \rho_nP_{c_ic_j}\right) W(\phi_{ij}, \beta_0; w_n) \right| }{w_n\rho_n|\E_k|^\alpha n^{2-\alpha}} > \frac{\delta}{2} \right\}\\
\leq & K \prb\left( \frac{|\E_k|^{2-\alpha}M_\phi M_\beta \epsilon}{\rho_n n^{2-\alpha}} \geq \frac{\delta}{2} \right) + 2K |B_\epsilon| \exp\left\{ -(n-1)w_n^2\rho_n^2\delta^2/4 \right\}\\
\leq & 2K\left( \frac{8M_\phi M_\beta \pi_0^{2-\alpha}\sqrt{p}}{\rho_n\delta} + 3 \right)^p\exp\left\{ -(n-1)w_n^2\rho_n^2\delta^2/4 \right\}
\end{align*}
Finally take a union bound over all possible community assignment $e$'s, we have
\begin{align*}
\prb\left( \max_{e,\beta}\frac{|R(e, \beta; w_n) - R^0(e, \beta; w_n)|}{
w_n\rho_n n^{2-\alpha}} > K\delta \right) & \leq 2K^{n+1}\left( \frac{8M_\phi M_\beta \pi_0^{2-\alpha}\sqrt{p}}{\rho_n\delta} + 3 \right)^p\exp\left\{ -(n-1)w_n^2\rho_n^2\delta^2/4 \right\}\\
&\leq C_1 \exp\left[ -nw_n^2\rho_n^2\delta^2/8 + n\log K + p\log\{ 1/(\rho_n \delta) \} \right]
\end{align*}
where $C_1:=2K\{ 8M_\phi M_\beta \pi_0^{2-\alpha}\sqrt{p} + 3\vee(\rho_n\delta) \}$. We always set $\rho_n\leq 1$ and will let $\delta\to 0$, so for large enough $n$, $C_1$ is a constant. Taking $\delta = 1/\sqrt{w_n\rho_n}$, the proof of Lemma \ref{lemma_1} is complete.
\end{proof}

We now proceed to studying the ``population version criterion'' $R^0$. Define $U, D\in\mathbb{R}^{K\times K}$ such that $U_{kl} = \sum_{i=1}^n 1[e_i=k, c_i=l]/n$ and $D_{kl} = \pi_l$ if $k=l$ and $D_{kl}=0$ if $k\neq l$, where $\pi_l:=\sum_{i=1}^n 1[c_i=l]/n$. Roughly speaking, $U_{kl}$ is the proportion of nodes that belong to the $k$th estimated community and the $l$th true community, $\pi_l$ is the proportion of nodes that belong to the $l$th true community, and $U=D$ means the estimation is perfect. Define the unweighted criterion:
\begin{equation*}
  g(U):=\sum_{k=1}^K\frac{\sum_{l=1}^K \sum_{l'=1}^K U_{kl}U_{kl'}P_{ll'}}{ \left(\sum_{a=1}^K U_{ka}\right)^\alpha }
\end{equation*}
Each estimated community assignment $e$ induces a unique $U$, we write such $U$ as $U(e)$. It is easy to verify that
\begin{equation*}
  g\left(U(e)\right) = \sum_{k=1}^K\frac{\sum_{i,j\in\E_k} P_{c_ic_j}}{|\E_k|^\alpha n^{2-\alpha}}
\end{equation*}

\begin{lemma}\label{lemma_2}
Under conditions 1 and 2, there exists a constant $C_2$ such that
\begin{equation*}
  \max_{e,\beta} \left| \frac{R^0(e, \beta; w_n)}{w_n\rho_nn^{2-\alpha}} - g\left(U(e)\right) \right| \leq \frac{C_2}{w_n}
\end{equation*}
\end{lemma}
\begin{proof}[of Lemma~\ref{lemma_2}]
By definition, we have
\begin{align*}
& \max_{e, \beta}\left| \frac{R^0(e, \beta; w_n)}{w_n\rho_nn^{2-\alpha}} - g\left(U(e)\right) \right| = \max_e\sum_{k=1}^K \max_{\beta_k} \sum_{i,j\in\E_k} P_{c_ic_j} \frac{\ep[\exp(-\langle \phi_{ij}, \beta_k \rangle)]}{|\E_k|^\alpha w_n n^{2-\alpha}}\\
\leq & \max_e\sum_{k=1}^K \sum_{i,j\in\E_k} \frac{\exp(M_\phi M_\beta)}{|\E_k|^\alpha w_n n^{2-\alpha}} \leq \frac{K \exp(M_\phi M_\beta)}{w_n\pi_0^{2-\alpha}} = \frac{C_2}{w_n}
\end{align*}
where $C_2:=\frac{K \exp(M_\phi M_\beta)}{\pi_0^{2-\alpha}}$, and the two inequalities are due to conditions \ref{condition_1} and \ref{condition_2} respectively.
\end{proof}

\begin{lemma}\label{lemma_3}
Under condition \ref{condition_3}, choosing $\alpha\in \left(\max_{1\leq k<l\leq K} 2(K-1)P_{kl}/\min(P_{kk}, P_{ll}), 1\right)$, for all $U$ satisfying $\sum_{k=1}^K U_{kl} = \pi_l$ for all $1\leq k\leq K$ we have that $g(U)$ is uniquely maximized at $U=D$, where recall that $D:=\textrm{diag}(\pi_1,\ldots,\pi_K)$.
\end{lemma}

\begin{proof}[of Lemma~\ref{lemma_3}]
We have
\begin{align}
& g(D) - g(U) = \sum_{l=1}^K \left(\sum_{k=1}^K U_{kl}\right)^{2-\alpha} P_{ll'} - \sum_{k=1}^K\frac{ \sum_{l=1}^K U_{kl}^2 P_{ll} + \sum_{l=1}^K\sum_{l'\neq l}U_{kl}U_{kl'}P_{ll'} }{\left(\sum_{a=1}^K U_{ka}\right)^\alpha}\nonumber\\
=&\sum_{l=a}^K\left\{ \left( \sum_{k=1}^K U_{kl} \right)^{2-\alpha} - \sum_{k=1}^K \frac{U_{kl}^2}{\left(\sum_{a=1}^K U_{ka}\right)^\alpha} \right\} P_{ll} - \sum_{k=1}^K\sum_{l=1}^K\sum_{l'\neq l}\left\{ \frac{U_{kl}U_{kl'}}{\left(\sum_{a=1}^K U_{ka}\right)^\alpha} \right\} P_{ll'} \label{diff_gD_gU}
\end{align}
For $0<\alpha<1$, since $U_{kl}$ is nonnegative for any $k, l$, we have $\left( \sum_{k=1}^K U_{kl} \right)^{2-\alpha} \geq \sum_{k=1}^K U_{kl}^{2-\alpha}$. By mid-value theorem, there exists $\xi_{kl}\in\left(0, \sum_{a\neq l}U_{ka}\right)$, such that $\left( \sum_{a=1}^K U_{ka} \right)^\alpha - U_{kl}^\alpha = \alpha\left( \sum_{a\neq l}U_{ka} \right) / \left(U_{kl} + \xi^{kl}\right)^{1-\alpha} \geq \alpha\left( \sum_{a\neq l}U_{ka} \right) / \left( \sum_{a=1}^K U_{ka} \right)^{1-\alpha}$. The final preparation before lower bounding \eqref{diff_gD_gU} is the following fact. For $0<\alpha<1$ and $x, y\geq 0$ satisfying $x+y\leq u$, we have
\begin{equation}
x^{2-\alpha}(u-x) + y^{2-\alpha}(u-y)\geq x y u^{1-\alpha} \label{claim_xyu}
\end{equation}
To show \eqref{claim_xyu}, divide its left hand side by $u^{3-\alpha}$, we have
\begin{align*}
&\frac{x^{2-\alpha}(u-x) + y^{2-\alpha}(u-y)}{u^{3-\alpha}} = \left(\frac{x}{u}\right)^{2-\alpha} \left(1-\frac{x}{u}\right) + \left(\frac{y}{u}\right)^{2-\alpha} \left(1-\frac{y}{u}\right) - \frac{xy}{u^2}\\
\geq & \left(\frac{x}{u}\right)^2 \left(1-\frac{x}{u}\right) + \left(\frac{y}{u}\right)^2 \left(1-\frac{y}{u}\right) - \frac{xy}{u^2} = \left\{ \left(\frac{x}{u}\right)^2 + \left(\frac{y}{u}\right)^2 - \frac{xy}{u^2} \right\}\left(1-\frac{x+y}{u}\right)\geq 0
\end{align*}
We now lower bound the first term on the right hand side of \eqref{diff_gD_gU}.
\begin{align}
&\sum_{l=a}^K\left\{ \left( \sum_{k=1}^K U_{kl} \right)^{2-\alpha} - \sum_{k=1}^K \frac{U_{kl}^2}{\left(\sum_{a=1}^K U_{ka}\right)^\alpha} \right\} P_{ll} = \sum_{l=1}^K\sum_{k=1}^K\frac{ U_{kl}^{2-\alpha}\left\{ \left(\sum_{a=1}^K U_{ka}\right)^\alpha - U_{kl}^\alpha \right\} }{\left(\sum_{a=1}^K U_{ka}\right)^\alpha}P_{ll}\nonumber\\
\geq & \sum_{l=1}K\sum_{k=1}^K \frac{U_{kl}^{2-\alpha}\left(\sum_{a\neq l}U_{ka}\right)}{\sum_{a=1}^K U_{ka}} \alpha P_{ll}\geq \sum_{l=1}K\sum_{k=1}^K \frac{U_{kl}^{2-\alpha}\left(\sum_{a\neq l}U_{ka}\right)}{\sum_{a=1}^K U_{ka}} \sum_{l'\neq l} 2P_{ll'}\nonumber\\
=& \sum_{k=1}^K\left\{ \sum_{l=1}^K\sum_{l'\neq l} \frac{U_{kl}^{2-\alpha}\left(\sum_{a\neq l} U_{ka}\right) P_{ll'}}{\sum_{a=1}^K U_{ka}}  +  \sum_{l'=1}^K\sum_{l\neq l'} \frac{U_{kl'}^{2-\alpha}\left(\sum_{a\neq l'} U_{ka}\right) P_{ll'}}{\sum_{a=1}^K U_{ka}}  \right\}\nonumber\\
=& \sum_{k=1}^K \sum_{l=1}^K\sum_{l'\neq l} \frac{U_{kl}^{2-\alpha}\left(\sum_{a\neq l}U_{ka}\right) + U_{kl'}^{2-\alpha}\left(\sum_{a\neq l'} U_{ka}\right)}{\sum_{a=1}^K U_{ka}} P_{ll'}      \geq \sum_{k=1}^K\sum_{l=1}^K\sum_{l'\neq l} \frac{U_{kl}U_{kl'}}{\left(\sum_{a=1}^K U_{ka}\right)^\alpha}P_{ll'}   \label{bound_first_term_diff_gD_gU}
\end{align}
where to obtain the last equality we applied \eqref{claim_xyu} with $x=U_{kl}$, $y=U_{kl'}$ and $u = \sum_{a=1}^K U_{ka}$. Plugging \eqref{bound_first_term_diff_gD_gU} into \eqref{diff_gD_gU}, we have
\begin{equation*}
g(D) - g(U)\geq 0
\end{equation*}
where it is easy to see equality holds when and only when $U=D$.
\end{proof}

\begin{proof}[Proof of the Main Theorem]
Denote $\hat{e}:=\arg\max_e\left(\max_\beta R(e, \beta; w_n)\right)$. By Lemma \ref{lemma_1} and Lemma \ref{lemma_2}, we have
\begin{equation}
\max_{e,\beta}\left|\left\{\frac{R(e, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} - g\left(U(e)\right)\right\} \right| = O_p\left(\frac{1}{\sqrt{w_n\rho_n}}\right)    \label{diff_R_gU}
\end{equation}
It is easy to verify that $2\|e-c\|_1/n=\|U(e)-D\|_1$ for any $e$, where for $Q\in \mathbb{R}^{K\times K}$ we define $\|Q\|_1:=\sum_{k=1}^K\sum_{l=1}^l |Q_{kl}|$, therefore it suffices to bound $\|U(\hat{e})-D\|_1$.

For any sequence of decreasing positive numbers $\{x_n\}$ that $x_n\to 0$, define $y_n:=\sup_{U: g(D) - g(U)\leq x} \|U-D\|_1$. It is easy to see that $y_n$ is non-increasing. Also $y_n$ converges to $0$. Otherwise we have $\sup_{U: \|U-D\|_1\geq \lim_{n\to \infty}y_n}g(U) = g(D)$ by the compactness of the domain of $U$ and the continuity of $g$. This contradicts Lemma \ref{lemma_3}.
Now choose $x_n$ such that $x_n\to 0$ and $\sqrt{w_n\rho_n}x_n\to\infty$, then by \eqref{diff_R_gU}, we have
\begin{align}
\prb\left[  \left\{ \left|\frac{R(\hat{e}, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} - g\left(U(\hat{e})\right) \right| > \frac{x_n}{2} \right\} \bigcup \left\{ \left|\frac{R(c, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} - g\left(D\right) \right| > \frac{x_n}{2} \right\} \right]\to 0      \label{sample_approach_pop}
\end{align}
and the event inside the probability of \eqref{sample_approach_pop} implies
\begin{equation*}
g(D) - g\left(U(\hat{e})\right) \leq \frac{R(c, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} - \frac{R(\hat{e}, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} + x_n \leq x_n
\end{equation*}
and therefore $2\|\hat{e}-c\|_1/n=\|U(\hat{e})-D\|_1\leq y_n$. Since $y_n\to 0$, the proof of the Main Theorem is complete.
\end{proof}










==> texsections/proof_backup.tex <==
We start with definining notation. Let $\E_k$ denote the set of nodes belonging to the $k$th estimated community and ${\cal C}_k$ denote the node set of the $k$th true community. Then by definition $e=\{{\cal E}_1, \ldots, \E_k\}$ and $c=\{{\cal C}_1,\ldots, {\cal C}_K\}$. We set $w_{\max}$ to depend on $n$, and therefore denote it as $w_n$ for convenience. Let $S_k(e, \beta_k; w_n) := \sum_{i, j\in \E_k}A_{ij} w(\phi_{ij}, \beta_k; w_n)$ be the sum of weighted edges in community $k$. Also define the population versions of $S_k$ as follows: $S_k^A(e, \beta_k; w_n) := \sum_{i, j\in \E_k} \rho_n P_{c_ic_j}w(\phi_{ij}, \beta_k; w_n)$ and $S_k^0(e, \beta_k; w_n) := \sum_{i, j\in \E_k} \rho_n P_{c_ic_j} \mathbb{E}[w(\phi_{ij}, \beta_k; w_n)]$. The expectation in $S_k^0$ is taken on random node features. Then the joint community detection criterion can be rewritten as:
\begin{equation*}
	R(e, \beta; w_n) = \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} A_{ij}w(\phi_{ij}, \beta_k; w_n) = \sum_{k=1}^K\frac{S_k(e, \beta_k; w_n)}{|\E_k|^\alpha}
\end{equation*}
Also define its population versions:
\begin{align*}
	R^A(e, \beta; w_n) &:= \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} \rho_n P_{c_ic_j}w(\phi_{ij}, \beta_k; w_n) = \sum_{k=1}^K\frac{S_k^A(e, \beta_k; w_n)}{|\E_k|^\alpha}\\
	R^0(e, \beta; w_n) &:= \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} \rho_n P_{c_ic_j}\mathbb{E}[w(\phi_{ij}, \beta_k; w_n)] = \sum_{k=1}^K\frac{S_k^0(e, \beta_k; w_n)}{|\E_k|^\alpha}
\end{align*}

\begin{lemma}\label{lemma_1}
Under conditions \ref{condition_1} and \ref{condition_2}, we have
\begin{align*}
	\mathbb{P}\left\{ \max_{e, \beta} \sum_k\frac{|X_k(e, \beta; w_n)|}{w_n\rho_n |\E_k|^\alpha n^{2-\alpha}} > 3K\epsilon \right\} &\leq 2K^{n+1}\left( \frac{2M_\beta^2 M_\phi\sqrt{p}}{\epsilon\rho_n} \right)^p \exp\left( -\frac{\frac{1}{8}\rho_n^2\pi_0^{\alpha}n^2\epsilon^2}{1+\frac{1}{6}\rho_n\epsilon} \right)\\
& + 2K^{n+1}\left( \frac{2M_\beta^2 M_\phi\sqrt{p}}{\epsilon\rho_n} \right)^p \exp\left\{ -(n-1)\epsilon^2 \right\}
%2\left( \frac{2M_\beta M_\phi\sqrt{p}}{\epsilon\rho_n \pi_0^{2-\alpha}} \right)^p K^{n+1} \exp\left( -\frac{\frac{1}{8}\rho_n^2\pi_0^{2\alpha}n^2\epsilon^2}{1+\frac{1}{6}\rho_n\pi_0^{2-\alpha}\epsilon} \right)\\
%	& + 2\left( \frac{2M_\beta M_\phi \sqrt{p}}{\epsilon\pi_0^{2-\alpha}} \right)^p K^{n+1} \exp\left( -\frac{\pi_0^{2\alpha}nw_n^2\epsilon^2}{4e^{2M_\beta M_\phi}} \right)
\end{align*}
where $p$ is the dimension of $\phi$ and $\beta$.
\end{lemma}

\begin{proof}[of Lemma~\ref{lemma_1}]
Define $ X_{k}^A(e, \beta; w) := S_{k}(e, \beta; w) - S_{k}^A(e, \beta; w)$, $X_{k}^0(e, \beta; w) := S_{k}^A(e, \beta; w) - S_{k}^0(e, \beta; w)$ and $X_{k}(e, \beta; w) := X_{k}^A(e, \beta; w) + X_{k}^0(e, \beta; w)$. First we fix $e$ and $\beta$. For any $k$, by Bernstein's inequality, we have
\begin{align*}
	& \pr\left\{ \frac{|X_k^A(\ebkw)|}{w_n\rho_n\eka n^{2-\alpha}} > \frac{\epsilon}{2} \right\} = \pr\left\{ \frac{\Big| \sum_{i, j\in \E_k} (A_{ij}-\rho_n P_{c_ic_j})w_{ij} \Big|}{w_n\rho_n\eka n^{2-\alpha}} > \frac{\epsilon}{2} \right\}\\
\leq & 2\exp\left\{ -\frac{ \frac{1}{2}\left( \frac{1}{2}w_n\rho_n|\E_k|^\alpha n^{2-\alpha}\epsilon \right)^2 }{ w_n^2|\E_k|^2 + \frac{1}{3}w_n \left( \frac{1}{2}w_n\rho_n|\E_k|^\alpha n^{2-\alpha}\epsilon \right)} \right\}
%\leq  2\exp\left( -\frac{\frac{1}{8}\rho_n^2|\E_k|^{2\alpha}n^{4-2\alpha}\epsilon^2}{n^2+\frac{1}{6}\rho_n\eka n^{2-\alpha}\epsilon} \right) 
\leq 2\exp\left( -\frac{\frac{1}{8}\rho_n^2\pi_0^{\alpha}n^2\epsilon^2}{1+\frac{1}{6}\rho_n\epsilon} \right)
\end{align*}
where the last inequality used the fact that $|\E_k|^2\leq |\E_k|^\alpha n^{2-\alpha}$ and Condition \ref{condition_2}.
Then we establish the uniform bound over all $\beta_k$'s, with $e$ still keep fixed. Consider an $\epsilon$-net $B_\epsilon$ of $[-M_\beta, M_\beta]^p$, which is the domain of $\beta_k$(recall that $p$ is the number of node features). For each dimension we split $[-M_\beta, M_\beta]$ into intervals of length $(\rho_n\epsilon)/(2M_\phi M_\beta \sqrt{p})$. Then the size of the $\epsilon$-net is $\left\{ 2M_\phi M_\beta^2\sqrt{p}/(\rho_n\epsilon) \right\}^p$. For any $\beta_k$, let $\beta(\beta_k, B_\epsilon)\in B_\epsilon$ be the best approximation to $\beta_k$ in the $\epsilon$-net. Then for any node pair $(i, j)$ and any $k$, by Condition \ref{condition_1}, we have 
\begin{align*}
&\max_{\beta_k}|w(\phi_{ij}, \beta_k; w_n) - w(\phi_{ij}, \beta(\beta_k, B_\epsilon); w_n)| \leq \max_\beta |\frac{\partial w(\phi_{ij}, \beta; w_n)}{\partial \beta}| |\beta_k - \beta(\beta_k, B_\epsilon)|\\
\leq& M_\phi M_\beta \exp(M_\phi M_\beta) \frac{\rho_n\epsilon}{2M_\phi M_\beta} \leq \frac{w_n\rho_n\epsilon}{2}
\end{align*}
Therefore,
\begin{align*}
	\max_{\beta_k}\frac{ |X_k^A(e,\beta_k;w_n) - X_k^A(e,\beta_\epsilon(\beta_k);w_n)| }{ w_n\rho_n |\E_k|^\alpha n^{2-\alpha} } \leq \frac{|\E_k|^2 \max_{ij} \max_{\beta_k} |w(\phi_{ij}, \beta_k; w_n) - w(\phi_{ij}, \beta(\beta_k, B_\epsilon); w_n)|}{w_n\rho_n |\E_k|^\alpha n^{2-\alpha}}\leq \frac{\epsilon}{2}
% \frac{ |\E_k|^2 M_\phi w_n \left( \frac{\pi_0^{2-\alpha}\epsilon \rho_n}{2M_\phi} \right) }{ w_n\rho_n |\E_k|^\alpha n^{2-\alpha} } = \frac{\epsilon}{2}
\end{align*}
Therefore,
\begin{align*}
	\mathbb{P}\left( \max_{\beta_k} \frac{ |X_k^A(\ebkw)| }{w_n\rho_n\eka n^{2-\alpha}} > \epsilon \right) &\leq \mathbb{P}\left( \max_{\beta_k\in B_\epsilon} \frac{ |X_k^A(\ebkw)| }{w_n\rho_n\eka n^{2-\alpha}} > \frac{\epsilon}{2} \right)\\
	& + \mathbb{P}\left( \max_{\beta_k} \frac{ |X_k^A(e,\beta_k;w_n) - X_k^A(e,\beta_\epsilon(\beta_k);w_n)| }{ w_n\rho_n |\E_k|^\alpha n^{2-\alpha} } > \frac{\epsilon}{2} \right)\\
 	& \leq 2\left( \frac{2M_\beta^2 M_\phi\sqrt{p}}{\epsilon\rho_n} \right)^p \exp\left( -\frac{\frac{1}{8}\rho_n^2\pi_0^{\alpha}n^2\epsilon^2}{1+\frac{1}{6}\rho_n\epsilon} \right)  
\end{align*}

Summing over $K$ communities and taking maximum over $e$ yields
\begin{equation}
 \mathbb{P}\left( \max_{e, \beta} \sum_k \frac{ |X_k^A(\ebkw)| }{w_n\rho_n\eka n^{2-\alpha}} > K\epsilon \right) \leq 2K^{n+1}\left( \frac{2M_\beta^2 M_\phi\sqrt{p}}{\epsilon\rho_n} \right)^p \exp\left( -\frac{\frac{1}{8}\rho_n^2\pi_0^{\alpha}n^2\epsilon^2}{1+\frac{1}{6}\rho_n\epsilon} \right)    \label{lemma1_eqn1}
\end{equation}


We then bound $X_k^0$'s. By Hoeffding's inequality \citep{hoeffding1963probability}, for fixed $e$ and $\beta$, we have
\begin{align*}
	&\pr\left( \frac{ |X_k^0(\ebkw)| }{w_n\rho_n \eka n^{2-\alpha}} >\epsilon \right) = \pr\left( \frac{ |\sum_{i, j\in \E_k}P_{c_ic_j}(w_{ij} - E[w_{ij}])| }{ |\E_k|^2 } > \frac{w_n n^{2-\alpha} \epsilon}{|\E_k|^{2-\alpha}} \right)\\
	\leq & 2\exp\left\{ -2\frac{[n/2] \left( \frac{ w_n n^{2-\alpha} \epsilon}{|\E_k|^{2-\alpha}} \right)^2 }{ w_n^2 } \right\}\leq 2\exp\left\{ -(n-1)\epsilon^2 \right\}
% 2\exp\left( -\frac{2\left[\frac{n}{2}\right]\pi_0^{2\alpha}\epsilon^2}{\left(\frac{2e^{M_\beta M_\phi}}{w_n}\right)^2} \right) = 2\exp\left( -\frac{\pi_0^{2\alpha}nw_n^2\epsilon^2}{4e^{2M_\beta M_\phi}} \right)
\end{align*}
To obtain the uniform bound over $\beta$, we introduce the same $\epsilon-$net as in the previous part of the proof and follow the same trick. We have:
\begin{equation}
	\pr\left( \max_{e, \beta} \sum_k\frac{|X_k^0(\ebkw)|}{w_n\rho_n\eka n^{2-\alpha}} > 2K\epsilon \right) \leq 2K^{n+1}\left( \frac{2M_\beta^2 M_\phi\sqrt{p}}{\epsilon\rho_n} \right)^p \exp\left\{ -(n-1)\epsilon^2 \right\}  \label{lemma1_eqn2}
\end{equation}

Combining equations \eqref{lemma1_eqn1} and \eqref{lemma1_eqn2} yields the lemma.

% 
% By Bernstein's inequality,
% \begin{align*}
% 	\pr\left( \frac{X_k^A(\ebkw)}{w_n\rho_n\eka n^{2-\alpha}} > \frac{\epsilon}{2} \right) &= \pr\left( \frac{\Big| \sum_{i, j\in \E_k} (A_{ij}-P_{c_ic_j})w_{ij} \Big|}{w_n\rho_n\eka n^{2-\alpha}} > \frac{\epsilon}{2} \right)\\
% 	&\leq 2\exp\left( -\frac{\frac{1}{8}\rho_n^2|\E_k|^{2\alpha}n^{4-2\alpha}\epsilon^2}{n^2+\frac{1}{3}\rho_n\eka n^{2-\alpha}} \right)\\
% 	&\leq 2\exp\left( -\frac{\frac{1}{8}\rho_n^2\pi_0^{2\alpha}n^2\epsilon^2}{1+\frac{1}{3}\rho_n} \right)
% \end{align*}
% Consider an $\epsilon$-net named $B_\epsilon$ for $\beta$. Split the interval $[-M_\beta, M_\beta]$ into grids with side $\frac{\epsilon}{2\sqrt{p}}$, then the size of the $\epsilon$-net is $|B_\epsilon|=\left(\frac{M_\beta}{\epsilon/(2\sqrt{p})}\right)^p = (2M_\beta \sqrt{p})^p\epsilon^{-p}$. We then have
% \begin{align*}
% 	&\pr\left( \max_{\beta_k} \frac{\Big| X_k^A(\ebkw) \Big|}{|\E_k|^2} >\epsilon \right)\\
% 	\leq & \pr\left( \max_{\beta_k} \frac{\Big| X_k^A(\ebkw) - X_k^A(e, \beta_\epsilon(\beta_k); w_n) \Big|}{|\E_k|^2} >\frac{\epsilon}{2} \right) + \pr\left( \max_{\beta\in B_\epsilon} \frac{\Big| X_k^A(e, \beta; w_n) \Big|}{|\E_k|^2} >\frac{\epsilon}{2} \right)\\
% 	\leq & 2(M_\beta\sqrt{p})^p \epsilon^{-p} \exp\left( -\frac{\frac{1}{8}|\E_k|^2 \epsilon^2}{1+\frac{1}{3}\epsilon} \right)
% \end{align*}
% where $\beta_\epsilon(\beta_k)\in B_\epsilon$ is defined to be the element of $B_\epsilon$ closest to $\beta_k$. Taking maximum over $e$ yields:
% \begin{align*}
% 	\pr\left( \max_{e, \beta} \sum_k\frac{\Big| X_k^A(\ebkw) \Big|}{|\E_k|^2} > K\epsilon \right) \leq 2(M_\beta\sqrt{p})^p\epsilon^{-p}K^(n+1)\exp\left( -\frac{\frac{1}{8}|\E_k|^2 \epsilon^2}{1+\frac{1}{3}\epsilon} \right)
% \end{align*}
% Then by noticing that $|\E_k|\geq \pi_0 n$ we have
% \begin{equation}
% 	\pr\left( \max_{e, \beta} \sum_k\frac{\Big| X_k^A(\ebkw) \Big|}{\rho_n\eka n^{2-\alpha}} > K\epsilon \right) \leq 2(M_\beta\sqrt{p})^p\epsilon^{-p}K^(n+1)\exp\left( -\frac{\frac{1}{8}\pi_0^{2\alpha}n^{4-2\alpha}\rho_n^2 \epsilon^2}{1+\frac{1}{3}\rho_n\epsilon} \right)  
% \end{equation}
% 
% We then bound $X_k^0$'s. By Hoeffding's inequality, for fixed $e$ and $\beta$, we have
% \begin{align*}
% 	\pr\left( \frac{X_k^0(\ebkw)}{\eka n^{2-\alpha}} >\epsilon \right) &= \pr\left( \frac{\sum_{i, j\in \E_k}P_{c_ic_j}(w_{ij} - E[w_{ij}])}{\eka n^{2-\alpha}} < \epsilon \right)\\
% 	&\leq 2\exp\left( -\frac{2\left[\frac{n}{2}\right]\pi_0^{2\alpha}\epsilon^2}{\left(\frac{2e^{M_\beta M_\phi}}{w_n}\right)^2} \right)\\
% 	&= 2\exp\left( -\frac{\pi_0^{2\alpha}nw_n^2\epsilon^2}{4e^{2M_\beta M_\phi}} \right)
% \end{align*}
% By following the similar technique in the first part of the proof, 

\end{proof}



\begin{lemma}\label{lemma_2}
Under condition \ref{condition_3}, and if $P_{kl}<\min(P_{kk}, P_{ll})$ for $k\neq l$, we have
\begin{equation*}
	\max_\beta R_0(c, \beta; w_n) \geq \max_\beta R_0(e, \beta; w_n)
\end{equation*}
for all $e$.
\end{lemma}



\begin{proof}[of Lemma~\ref{lemma_2}]
Let $U_{kl}$ be the proportion of nodes that are estimated to belong to communtiy $k$ while truly belonging to community $l$. Then we have $\sum_k U_{kl} = \pi_l$, where $\pi_l$ is the true proportion of nodes in community $l$, and $|\E_k|/n=\sum_{a'}U_{ka'}$. Define $\mathbb{U}\in \mathbb{R}^{K\times K}$ whose $(k, l)$ element is $U_{kl}$ and $\mathbb{D}:=diag(\pi_1, \ldots, \pi_K)$. Define the rescaled continuous version of $R^0$, denoted by $\tilde{R}^0$, as follows: 
\begin{align*}
	\tilde{R}_0(U, \beta; w_n)&  := \sum_k \frac{1}{(\sum_{a'}U_{ka'})^\alpha}\sum_{ll'}U_{kl}U_{kl'}\mathbb{E}[w(\phi_{ll'}, \beta;w_n)]P_{ll'} / w_n\\
					& = \sum_k\frac{ \sum_{ll'} U_{kl} U_{kl'}\left[1-\frac{\mathbb{E}\{\exp(-\langle \phi_{ij},\beta_k \rangle)\}}{w_n}\right] P_{ll'} }{(\sum_{a'}U_{ka'})^\alpha}
\end{align*}
Then $\frac{R_0(e, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} = \tilde{R}_0\left( \left( \frac{|E_1|}{n}, \ldots, \frac{|\E_k|}{n} \right), \beta; w_n \right)$. We now show that $\mathbb{D}$ and its corresponding $\beta$ maximizes $\tilde{R}_0$. We start with proving for the case $\beta=0$.
\begin{align*}
	& \frac{w_n}{w_n-1}\left(\tilde{R}_0(\mathbb{D}, 0; w_n) - \tilde{R}^0(\mathbb{U}, 0; w_n)\right) = \sum_l \pi_l^{2-\alpha}P_{ll} - \sum_k\frac{1}{(\sum_l U_{kl})^\alpha}\sum_{ll'}U_{kl}U_{kl'}P_{ll'}\\
	=& \sum_l\left((\sum_k U_{kl})^{2-\alpha} - \sum_k\frac{U_{kl}^2}{(\sum_{a}U_{ka})^\alpha}\right)P_{ll} - \sum_{l, l', l\neq l'}\left( \sum_k\frac{U_{kl}U_{kl'}}{(\sum_{a}U_{ka})^\alpha} \right)P_{ll'}=:Q_1-Q_2
\end{align*}
Where $Q_1$ and $Q_2$ represent the two terms. For $0<\alpha<1$, $(\sum_k U_{kl})^{2-\alpha}\geq \sum_k U_{kl}^{2-\alpha}$, so we can lower bound $I_1$ by:
\begin{align*}
Q_1 &\geq \sum_l\left( \sum_k U_{kl}^{2-\alpha} - \sum_k\frac{U_{kl}^2}{(\sum_a U_{ka})^\alpha} \right)P_{kl} = \sum_l\sum_k \frac{U_{kl}^{2-\alpha}\left( (\sum_a U_{ka})^\alpha - U_{kl}^\alpha \right)}{(\sum_a U_{ka})^\alpha}P_{ll}
\end{align*}
By mid-value theorem, there exists $\xi_{kl}\in(0, \sum_{b\neq l}U_{kl})$ such that $\sumka - U_{kl}^\alpha = \alpha(U_{kl}+\xi_{kl})^{\alpha-1}(\sum_{a\neq l}U_{ka}) \geq \alpha (\sum_a U_{ka})^{\alpha-1}(\sum_{a\neq l}U_{ka})$. Therefore,
\begin{align*}
	Q_1-Q_2 &\geq \sum_k\sum_l\frac{U_{kl}^{2-\alpha}\sum_{a\neq l}\uka}{\sum_a \uka} \alpha P_{ll} - \sum_k\sum_{l, l', l\neq l'}\frac{\ukl U_{kl'}}{\sumka}P_{ll'}\\
	&\geq \sum_k\left[ \sum_l\frac{\ukl^{2-\alpha}\sum_{a\neq l}U_{ka}}{\sum_a\uka}\left( 2\sum_{l'\neq l} P_{ll} \right) - \sum_{l, l', l\neq l'}\frac{\ukl U_{kl'}}{\sumka} P_{ll'} \right]\\
	&= \sum_k\sum_{l, l', l\neq l'} \left[ \frac{\ukl^{2-\alpha}\sum_{a\neq l}\uka + U_{kl'}^{2-\alpha}\sum_{a\neq l'}U_{kl'}}{\sum_a\uka} - \frac{\ukl U_{kl'}}{\sumka}\right] P_{ll'}\\
	&\geq \sum_k\sum_{l, l', l\neq l'}\left[ \frac{\ukl U_{kl'}(\sum_a\uka)^{1-\alpha}}{\sum_a \uka} - \frac{\ukl U_{kl'}}{\sumka} \right] P_{ll'} = 0
\end{align*}
The last inequality is due to the fact that for any $x, y\geq 0$, $x + y\leq u$, and $0<\alpha\leq 1$ we have
\begin{equation}
x^{2-\alpha}(u-x)+y^{2-\alpha}(u-y)\geq xyu^{1-\alpha}
\end{equation}
Indeed, letting $s:=x/u$, $t:=y/u$, then $v:=s+t\leq 1$. Dividing both sides by $u^{3-\alpha}$, we have:
\begin{align*}
	& (x^{2-\alpha}(u-x)+y^{2-\alpha}(u-y)- xyu^{1-\alpha})/u^{3-\alpha} = s^{2-\alpha}(1-s) + t^{2-\alpha}(1-t) - st\\
	\geq & s^2(1-(v-t)) + t^2(1-(v-s)) - st =(s^2+t^2-st)(1-v)\geq 0
\end{align*}
The last inequality is obtained by taking $x=\ukl$, $y=U_{kl'}$ and $u=\sum_a\uka$. This concludes the proof for the unweighted case (i.e. $\beta=0$).\\

%{\bf Claim} For $x, y>0$, $x + y\leq u$, and $0<\alpha\leq 1$ we have
%\begin{equation}
%x^{2-\alpha}(u-x)+y^{2-\alpha}(u-y)\geq 2xyu^{1-\alpha}
%\end{equation}
%\begin{proof}[Proof of Claim]
% Let $s:=x/u$, $t:=y/u$, dividing both sides by $st u^{3-\alpha}$, it suffices to show that
% $$
%	\left(\frac{s}{t}\right) s^{-\alpha}(1-s) + \left(\frac{t}{s}\right) t^{-\alpha}(1-t) \geq 2
% $$
% Then by the fact that $LHS\geq 2\sqrt{\left(\frac{s}{t}\right)s^{-\alpha}(1-s) \cdot \left(\frac{t}{s}\right)t^{-\alpha}(1-t)}\geq 2\sqrt{\frac{1-s}{s}\frac{1-t}{t}}\geq 2$, the claim is proved. Notice the equality is achieved only when $t=1-s$.
%\end{proof}
%
%By the claim, also recalling the assumption that $P_{ll'}\leq \alpha\min(P_{ll}, P_{l'l'})$ for $l\neq l'$, then the entire RHS of (\ref{star}) is lower bounded by
%\begin{align*}
%	RHS(\ref{star}) &\geq \sum_{k, l, l', l\neq l'} \alpha \left[ \frac{U_{kl}^{2-\alpha}\sum_{b\neq l}U_{kb} + U_{kl'}^{2-\alpha}\sum_{b\neq l'}U_{kb}}{\sum_{a}U_{ka}} - \frac{U_{kl}U_{kl'}}{(\sum_aU_{ka})^\alpha} \right]P_{ll'}\\
%	&\geq \sum_{l, l', l\neq l'}\alpha\left[ \frac{U_{kl}U_{kl'} (\sum_a U_{ka})^{1-\alpha}}{\sum_a U_{ka}} - \frac{U_{kl}U_{kl'}}{(\sum_aU_{ka})^\alpha} \right]P_{ll'} = 0
%\end{align*}
%

We then continue to prove Lemma 2, which is the weighted case. Let $\hat{\beta}:=\arg\max_\beta \tilde{R}^0(\mathbb{U}, \beta)$ and $\tilde{\beta}:=\arg\max_\beta \tilde{R}^0(\mathbb{D}, \beta)$. Since for all $l$, $\mathbb{E}[w(\phi_{ll}, \hat{\beta}_k;w_n)]\leq \mathbb{E}[w(\phi_{ll}, \tilde{\beta}_l;w_n)]$, and for $l\neq l'$, $\mathbb{E}[w(\phi_{ll'}, \hat{\beta}_k; w_n)]/w_n\leq 1-\mathbb{E}[e^{-\langle\phi_{ll'}, \hat{\beta}_k\rangle}]/w_n\leq 1-e^{-\mathbb{E}[\langle\phi_{ll'}, \hat{\beta}_k\rangle ]}/w_n\leq \mathbb{E}[w(\phi_{ll'}, 0;w_n)]/w_n=1-1/w_n$, since $\mathbb{E}[\phi_{ll'}]\leq 0$ for $l\neq l'$. Recall the notation that $\mathbb{E}[\phi_{ll'}]\leq 0$ means elemenet of $\mathbb{E}[\phi_{ll'}]$ is nonpositive. Therefore we have
\begin{align*}
& \tilde{R}^0(\mathbb{U}, \hat{\beta})w_n = \sum_{k=1}^K\frac{1}{\sumka} \sum_{l=1}^K\sum_{l'=1}^K U_{kl}U_{kl'}\mathbb{E}[w(\phi_{ll'}, \hat{\beta}_k; w_n)]P_{ll'}\\
\leq & \sum_{k=1}^K\frac{1}{\sumka}\sum_{l=1}^K U_{kl}^2 \mathbb{E}[w(\phi_{ll},\tilde{\beta}_l;w_n)]P_{ll} + \sum_{k=1}^K\frac{1}{\sumka}\sum_{l=1}^K\sum_{l'=1, l'\neq l}^K U_{kl}U_{kl'} \mathbb{E}[w(\phi_{ll'}, 0; w_n)] P_{ll'}\\
\leq & \sum_{k=1}^K \frac{1}{\sumka} \sum_{l=1}^K U_{kl}^2 \mathbb{E}[w(\phi_{ll}, \tilde{\beta}_l; w_n)]P_{ll} + \sum_l\left[ \pi_l^{2-\alpha} - \sum_k\frac{U_{kl}^2}{\sumka} \right] \mathbb{E}[w(\phi_{ll}, 0; w_n)] P_{ll}\\
\leq & \sum_{k=1}^K \frac{1}{\sumka} \sum_{l=1}^K U_{kl}^2 \mathbb{E}[w(\phi_{ll}, \tilde{\beta}_l; w_n)]P_{ll} + \sum_l\left[ \pi_l^{2-\alpha} - \sum_k\frac{U_{kl}^2}{\sumka} \right] \mathbb{E}[w(\phi_{ll}, \tilde{\beta}_l; w_n)] P_{ll}\\
= & \tilde{R}^0(\mathbb{D},\tilde{\beta})w_n
\end{align*}
Notice that for the last inequality we used the fact that $\pi_l^{2-\alpha}\geq \sum_k\frac{U_{kl}^2}{\left(\sum_a U_{ka}\right)^\alpha}$ for all $l$. Indeed,
$$
\sum_k\frac{U_{kl}^2}{\left(\sum_a U_{ka}\right)^\alpha}  \leq \sum_k U_{kl}^{2-\alpha} \leq \left(\sum_k U_{kl}\right)^{2-\alpha} =: \pi^{2-\alpha}
$$
The proof for Lemma \ref{lemma_2} is completed.
\end{proof}


\begin{proof}[of the Main Theorem]
When $w_n\to\infty$, we have
\begin{align*}
	\tilde{R}_0(\mathbb{U}, \beta; w_n) &= \frac{R_0(e, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} = \sum_k\frac{1}{(|\E_k|/n)^\alpha}\sum_{l, l'} \left( \frac{P_{ll'}|\{(i, j):c_i=l, c_j=l'\}|}{n^2}\mathbb{E}[w(\phi_{ll'}, \beta_k; w_n)] \right)\\
	&=\sum_k\frac{1}{\sumka}\sum_{ll'}\ukl U_{kl'}\left( 1-\frac{\mathbb{E}[e^{\langle \phi_{ll'}, \beta_k \rangle}]}{w_n} \right)
\end{align*}
Define $g(\mathbb{U}):=\sum_k\frac{1}{\sumka}\sum_{ll'}\ukl U_{kl'}P_{ll'}$. We have
\begin{align}
	\sup_\beta \left| \frac{R_0(e, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} - g(\mathbb{U}) \right| &\leq (\sum_a \uka)^{2-\alpha} \sum_{ll'}\frac{U_{kl}}{\sum_a\uka}\frac{U_{kl'}}{\sum_a\uka} \frac{e^{M_\phi M_\beta}}{w_n} \leq \frac{K^3 e^{M_\phi M_\beta}}{w_n} \label{main_theorem_convergence_R0}
\end{align}

%\begin{align}
% \tilde{R}_0(\mathbb{U}, \beta; w_n) &= \frac{R_0(e, \beta; w_n)}{w_n\rho_n n^{2-\alpha}} \to \sum_k\frac{1}{(\sum_{a'}U_{ka'})^\alpha}\sum_{ll'} U_{kl} U_{kl'}P_{ll'} =: g(U) \label{main_theorem_convergence_R0}
%\end{align}
%where we consider the variation of the population version criterion for any fixed set of $P_{kl}$'s -- thus they do not enter the argument of $g$. Also notice that the convergence in \eqref{main_theorem_convergence_R0} is uniform for all $\beta$ since all edge weights are uniformly bounded by $e^{M_\phi M_\beta}$. 
For any $\delta>0$, by Lemma 2, $\mathbb{D}$ is the unique maximizer of $g(\mathbb{U})$ for $\mathbb{U}$ ranging over a compact set, we have $\sup_{\mathbb{U}:\|\mathbb{U}-\mathbb{D}\|_F>\delta} g(\mathbb{U}) < g(\mathbb{D})$. Let $\epsilon(\delta):= g(\mathbb{D}) - \sup_{\mathbb{U}:\|\mathbb{U}-\mathbb{D}\|_F>\delta} g(\mathbb{U})$. Denote $(\hat{e}, \hat{\beta}):=\arg\max_{e,\beta} R(e, \beta; w_n)$, and $\tilde{\beta}:=\arg\max_\beta R_0(c, \beta; w_n)$. One can verify that the definition of $\hat{\beta}$ and $\tilde{\beta}$ matches those in the proof of Lemma 2, so we do not differentiate in notation here. Let $\hat{\mathbb{U}}$ be the $(U_{kl})$ corresponding to $\hat{e}$ and notice that $\mathbb{D}$ corresponding to $c$.\\

Now the event $I_0:=\{\|\hat{e} - c\|_1/n > \delta\}$ implies that at least one of the events $I_1$ to $I_4$, defined as follows, happens: 
\begin{align*}
I_1 &:= \left\{\frac{|R(\hat{e}, \hat{\beta}; w_n) - R_0(\hat{e}, \hat{\beta}; w_n)|}{w_n\rho_n n^{2-\alpha}}>\frac{\epsilon(\delta)}{4}\right\}, & I_2 := \left\{\Big|\frac{R_0(\hat{e}, \hat{\beta}; w_n)}{w_n\rho_n n^{2-\alpha}} - g(\hat{\mathbb{U}})\Big|>\frac{\epsilon(\delta)}{4}\right\},\\
I_3 &:= \left\{\frac{|R(c, \tilde{\beta}; w_n) - R_0(c, \tilde{\beta}; w_n)|}{w_n\rho_n n^{2-\alpha}}>\frac{\epsilon(\delta)}{4}\right\}, & I_4 := \left\{\Big|\frac{R_0(c, \tilde{\beta}; w_n)}{w_n\rho_n n^{2-\alpha}} - g(\mathbb{D})\Big|>\frac{\epsilon(\delta)}{4}\right\}
\end{align*}
By Lemma 1, $\mathbb{P}(I_1), \mathbb{P}(I_3) \to 0$. By \eqref{main_theorem_convergence_R0}, $\mathbb{P}(I_2)=\mathbb{P}(I_4) = 0$ for large enough $n$(notice that both $R_0$ and $g$ are non-random functions). Then $\mathbb{P}(I_0)\leq \mathbb{P}(I_1) + \mathbb{P}(I_2) + \mathbb{P}(I_3) + \mathbb{P}(I_4)\to 0$. The main theorem follows.



% By Lemma 1, $\mathbb{P}\left( \frac{|R(e, \beta; w_n) - R_0(e, \beta; w_n)|}{w_n\rho_n n^{2-\alpha}} > \frac{\epsilon(\delta)}{2} \right) \to 0$. Letting $n$ be large enough such that $|\tilde{R}_0(\mathbb{U}, \beta; w_n) - g(U)|\leq \frac{\epsilon(\delta)}{2}$, then we have that with a diminishing probability, $\|\arg\max_e(\max_\beta R(e,\beta;w_n)) - c\|_2/n < \delta$. The weak consistency follows.

% For any $\delta>0$, we have
% \begin{align*}
% &\mathbb{P}\left( |\arg\max_e(\max_\beta R(e, \beta; w_n))-c|/n>\delta \right)\leq \mathbb{P}\left( \sup_{e, \beta} \frac{X(e, \beta; w_n)}{\rho_n n^{2-\alpha}} > \frac{\delta}{2C} \right)\\
% \leq &2K(M_\beta\sqrt{p})^p\left(\frac{\delta}{2C}\right)^{-p}K^{n+1}\left[ \exp\left( -\frac{\frac{1}{8}\pi^{2\alpha}n^{4-2\alpha}\rho_n^2 \left(\frac{\delta}{4KC}\right)^2}{1+\frac{1}{3}\frac{\delta}{4KC}} \right) + \exp\left( -\frac{\pi_0^{2\alpha}nw_n^2 \left(\frac{\delta}{4KC}\right)^2}{4e^{2M_\beta M_\phi}} \right) \right]\\
% &\to 0
% \end{align*}
% as $n\to\infty$. The weak consistency follows.
\end{proof}


==> texsections/section_11.tex <==
Community detection is a fundamental problem in network analysis, which has been extensively studied in a number of domains -- see  \cite{korean1}, \cite{korean2}, \cite{schlitt2007current} for some examples of applications.  A number of approaches to community detection are based on probabilistic models for networks with communities, such as the stochastic block model \cite{Holland83}, the degree-corrected stochastic block model \cite{Karrer10}, and the latent factor models \cite{Hoff2007, Hoff2009}.  Other approaches work by optimizing a criterion measuring the strength of community structure in some sense and spectral approximations to such criteria.  Examples include normalized cuts \cite{shi00},  modularity \cite{Newman&Girvan2004}, \cite{NewmanPNAS}, and many variants of spectral clustering,  for example  \cite{ruan2007efficient}.

Many of the existing community detection methods focus on analyzing the network based on its adjacency matrix only.  However, we often have access to additional information on the nodes, which we will refer to as node features, and sometimes edges as well, e.g., \cite{steglich2006applying}, \cite{snijders2006new} \cite{hummon1990analyzing}.  In many networks the distribution of node features is correlated with community structure \cite{Jure_ego}, and thus a natural question is whether we can improve community detection by using the node features.   Several approaches have been proposed that assume a certain generative model\textcolor{cyan}{(certain generative models)} for the network and its features, including the network random effect model \cite{hoff2003random}, the embedding feature model \cite{Zanghi:2010:CBR:1774858.1774960}, the Bayesian probabilistic model \cite{Xu:2012:MAA:2213836.2213894}, the latent variable model \cite{RSSA:RSSA471}, the discriminative approach \cite{Yang:2009:CLC:1557019.1557120}, the latent multigroup membership graph model \cite{Jure_multiple_attr}, and the social circles model for ego networks \cite{Jure_ego}.   Most of these approaches were\textcolor{cyan}{(are)} designed to fit specific feature types, and their effectiveness depends heavily on the correctness of model specification.  Approaches that are not model-based include edge weighing by node feature similarity \cite{viennet2012community}, matrix factorization \cite{Zhu07combiningcontent}, attribute-structure mining \cite{Silva:2012:MAC:2140436.2140443} and SA-clustering \cite{Cheng:2011:CLA:1921632.1921638}.  Most methods in this category use all features \textcolor{cyan}{(+in)} the same way without considering\textcolor{cyan}{(discriminating)} which ones influence the community structure\textcolor{cyan}{(are correlated with the community structure)}, and lack the flexibility of balancing the information coming from network adjacency matrix and its node features\textcolor{cyan}{(the network structure and node features)}.   Including irrelevant node features may potentially lead to worse community detection, while selecting features that cluster strongly, which is in\textcolor{cyan}{(by)} itself a difficult problem in clustering, may not correspond to features that correlate with community structure.

In this paper, we propose a new joint community detection criterion that combines network edge information and node features. The idea is that by properly weighing edges according to feature similarities on their terminal nodes, the community structure in the network is enhanced and thus the detection is improved.  We learn which features are most helpful in identifying community structure from data, and allow for the possibility that having similar features may make nodes more or less likely to connect\textcolor{cyan}{(connect more strongly or weakly)}, thus allowing for both assortative- and disassortative-type behavior for each individual feature.  On an intuitive level,  our method looks for an agreement between clustering structures suggested by the two data sources, the adjacency matrix and the node features.  Once the community structure is estimated, we can formally select relevant node features via a permutation test, or we can alternatively achieve feature selection by using an $\ell_1$ penalty on the feature coefficients.  Numerical experiments on simulated and real examples show that our method performs well compared to methods that use either the network alone or the features alone for clustering.

%\textcolor{cyan}{Comparing to \cite{Jure_ego}, which also allows adjusting the impacts from different features on the community detection result and balancing them with the impact of the network structure, our method incorporates these flexibilities in a simpler and more explicit formulation. This enables asymptotic studies as well as statistical tests.}    {\bf[comparison to Lesc.?]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The rest of the paper is organized as follows. In Section 2 we clarify the concept of community as our estimation target and set up basic notation. In Section 3, we establish the joint community detection criterion by first proposing a new community criterion on weighted networks and then formulating edge weights as functions of node features. In Section 4, we discuss the properties of the joint community detection criterion. We first discuss the detection mechanism of the criterion with fixed edge weights, then fix the community assignments and discuss feature selection. In Section 5, we describe the optimization algorithm steps. In Section 6 and 7, we apply our method to artificial and real life data sets, discuss the impact and choices of tuning parameters and compare its performance with benchmark methods. Section 8 discusses state future work.


==> texsections/section_1__Yuan_Zhang____________2015-07-24_.tex <==
\dropcap{C}ommunity detection is a fundamental problem in network analysis, extensively studied in a number of domains -- see  \cite{korean1} and \cite{schlitt2007current} for some examples of applications.  A number of approaches to community detection are based on probabilistic models for networks with communities, such as the stochastic block model \cite{Holland83}, the degree-corrected stochastic block model \cite{Karrer10}, and the latent factor model \cite{Hoff2007}.  Other approaches work by optimizing a criterion measuring the strength of community structure in some sense or spectral approximations to such criteria.  Examples include normalized cuts \cite{shi00},  modularity \cite{Newman&Girvan2004, NewmanPNAS}, and many variants of spectral clustering, see for example \cite{qin2013regularized}.
%  \cite{ruan2007efficient}.
%% , Hoff2009

Many of the existing methods detect communities based only on the network adjacency matrix.  However, we often have additional information on the nodes (node features), and sometimes edges as well, for example, \cite{steglich2006applying}, \cite{snijders2006new} and \cite{hummon1990analyzing}.  In many networks the distribution of node features is correlated with community structure \cite{Jure_ego}, and thus a natural question is whether we can improve community detection by using the node features.   Several generative models for the network and its features have been proposed, including the network random effects model \cite{hoff2003random}, the embedding feature model \cite{Zanghi:2010:CBR:1774858.1774960}, the latent variable model \cite{RSSA:RSSA471}, the discriminative approach \cite{Yang:2009:CLC:1557019.1557120}, the latent multi-group membership graph model \cite{Jure_multiple_attr}, the social circles model for ego networks \cite{Jure_ego}, the communities from edge structure and node attributes (CESNA) model \cite{yang2013community}, the Bayesian Graph Clustering (BAGC) model \cite{xu2012model} and the topical communities and personal interest (TCPI) model \cite{hoang2014joint}.   Most of these models are designed for specific feature types, and their effectiveness depends heavily on the correctness of model specification.  Approaches that are not model-based include weighted combinations of the network and feature similarities \cite{viennet2012community, binkiewicz2014covariate}, attribute-structure mining \cite{Silva:2012:MAC:2140436.2140443}, simulated annealing clustering \cite{Cheng:2011:CLA:1921632.1921638}, and compressive information flow \cite{smith2014partitioning}.  Most methods in this category use all the features in the same way without determining which ones influence the community structure and which do not, and lack flexibility in how to balance the network information with the information coming from its node features, which do not always agree.   Including irrelevant node features can only hurt community detection by adding in noise, while selecting features that by themselves cluster strongly, which is in itself a difficult problem in clustering, may not correspond to features that correlate with the community structure present in the adjacency matrix.

In this paper, we propose a new joint community detection criterion that uses both the network adjacency matrix and the node features. The idea is that by properly weighing edges according to feature similarities on their end nodes, we strengthen the community structure in the network thus make it easier to detect.   Rather than using all available features in the same way,  we learn which features are most helpful in identifying the community structure from data.   Intuitively,  our method looks for an agreement between clusters suggested by two data sources, the adjacency matrix and the node features.  Numerical experiments on simulated and real examples show that our method performs well compared to methods that use either the network alone or the features alone for clustering, as well as to a number of benchmark joint detection methods.


==> texsections/section_22.tex <==
Our method is based on the intuition that communities are characterized by having more edges within themselves than between.   While this is certainly\textcolor{cyan}{[remove ``certainly''?]} not the only possible type of community structure, it is a very common one, and this intuition underlies many other methods for community detection, e.g., modularity \cite{NewmanPNAS}.   Our goal is to use such a community detection criterion based on the adjacency matrix alone, and then weigh edges according to their feature similarities to improve \textcolor{cyan}{(the)?} detection.   While many such criteria have been proposed, having a simple criterion linear in the adjacency matrix makes optimization much more feasible in our particular situation, as will become clear below.   Let $A$ denote the adjacency matrix with $A_{ij}=1$ if there is an edge between nodes $i$ and $j$ and $A_{ij}=0$ otherwise, or else an edge weight (our methods work the same way for weighted and unweighted networks).  Let $\bm{f}_i$ denote the $p$-dimensional feature vector of node $i$. Let $K$ be the number of communities we are looking for, and let $\bm{e}$ be a  vector of label assignment, with $e_i = k$, $k = 1, \dots, K$, if node $i$ belongs to community $k$.   Let  $E_k = \{i: e_i = k\}$, and let $|E_k|$ be the number of nodes in community $k$.  As a starting point for community detection,  we use\textcolor{cyan}{(We start with)} a very simple analogue of modularity, 
\begin{equation}
      R(e)=\sum_{k=1}^K \frac{1}{|E_k|^\alpha}\sum_{i, j\in E_k}A_{ij} \ , %w_{ij} 
     \label{marginal_criterion}
\end{equation}
which is then maximized over all possible assignments $e$.  Here $\alpha > 0$ is a tuning parameter, and rescaling by\textcolor{cyan}{(the rescaling factor)} $|E_k|^\alpha$ is designed to rule out trivial solutions that put\textcolor{cyan}{(solution that puts)} all nodes in the same\textcolor{cyan}{(one)} community.   This criterion can be shown to be consistent under the stochastic block model by checking the conditions of the general theorem of\textcolor{cyan}{(in)} \cite{Bickel&Chen2009}.  Note also that when $\alpha=2$, the criterion is approximately the sum of edge densities within communities, and when $\alpha=1$, the criterion is the sum of average ``within community'' degrees, which both are\textcolor{cyan}{[remove ``are'']} intuitively represent community structure.  



Next, we introduce feature-based edge weights which, ideally, should upweigh edges within communities and downweigh edges between them, thus enhancing the community structure in the observed network.  However, node features may not be perfectly correlated with community structure, different communities may be driven\textcolor{cyan}{(correlate with)[since we are not proposign a generative model]} by different features, as pointed out by \cite{Jure_ego}, and features themselves may be noisy.  Thus we need to learn the impact of\textcolor{cyan}{(correlation between)} different features on\textcolor{cyan}{(and different)} communities as well as balance the role\textcolor{cyan}{(impact)} of the\textcolor{cyan}{[remove ``the''?]} network information and node features in community detection.  This leads us to propose\textcolor{cyan}{(proposing)} a {\bf joint community detection criterion (JCDC)}, defined by 
\begin{equation}
	\max_{\bm{e}, \bm{\beta}} R(\bm{e}; \bm{\beta}):=\sum_{k=1}^K\frac{1}{|E_k|^\alpha}\sum_{i,j\in E_k}A_{ij}w(\bm{f}_i, \bm{f}_j; \bm{\beta}_k) \label{JCDC}
\end{equation}
where $\alpha$ is a tuning parameter chosen by the user, and $\bm{\beta}$ is the unkonwn vector of coefficients that controls the impact of each feature.  Note that each community has its own vector of coefficients, which allows for features playing different roles in different communities.   

For the sake of simplicity, we model the edge weight $w_{ij}$ as a function of the node features $\bm{f}_i$ and $\bm{f}_j$ via a $p$-dimensional vector of their similarity measures $\bm{\phi}_{ij} = \bm{\phi}(\bm{f}_i, \bm{f}_j)$, setting
\begin{align}
w(\bm{f}_i, \bm{f}_j; \bm{\beta}_k) = w(\bm{\phi}_{ij}; \bm{\beta}_k) \label{similarity_to_weights}
\end{align} 
 The choice of similarity measures in $\bm{\phi}$ depends on the type of $\bm{f_i}$ (for example, on whether the features are numerical or categorical) and is determined on a case by case basis;  the only important property similarity is that it assigns higher values to features that are more similar. To eliminate potential differences in units and scales, we standarize all $\bm{\phi}_{ij}$ along each feature dimension.

Finally, we choose a functional form for $w$.   This function should be increasing in ``overall similarity'' between nodes, and choosing a concave function facilitates optimization.  In this paper, we use the exponential function
\begin{equation}
w(\bm{\phi}_{ij}, \bm{\beta}_0):=w_{\max}-e^{-\langle \bm{\phi}_{ij},\bm{\beta}_0 \rangle}\label{weight_function}
\end{equation}
One can use other functions of similar shapes, for example, the logit exponential function, which we found empirically to perform similarly.   Note that \eqref{weight_function} depends on an additional  tuning parameter $w_{\max} > 1$, whose role is to balance the roles of $A$ and $F$ in community detection;  this will be discussed in detail in Sections \ref{sec:fixedbeta} and \ref{sec:tuning}.  


% 
% There have been numerous community detection criteria proposed in the literature. To determine which existing criterion or what type of potential new criterion fits our goal of joint detection well, we start with establishing two basic principles.\\
% 
% First, we restrict the criterion to be a linear function of edge weights. In general, a non-likelihood-based method models the edge weights as a function of the features on nodes involved with a set of parameters.  The curvature of the community detection criterion as a function of the parameters has a crucial impact on the difficulty or even feasibility of the corresponding optimization problem. A desirable combination of the community detection criterion and the modeled edge weight function yields a convex(or concave, depending on whether the criterion is to be minimized or maximized) function of the parameters. Therefore, it is natural to work with a criterion linear in edge weights and later choose the weight function to be convex/concave.\\
% 
% Second, we look for criterion that measures the community significance directly. In our methodology, the estimated community structure serves to guide the selection of node features. Comparing to cut measures, criteria that are functions of weights on within community edges utilize more information provided by the network structure, since we only consider weights on edges, not unconnected node pairs. This character is crucial when the network is sparse. Also, this principle will be important in future work where we extend our current methodology to overlapping community scenario. Criteria that measure and minimize the between community connections encounter difficulty in addressing the overlapping communities in both defining and quantifying the between community edges.\\
% 
% Our criterion is inspired by from a ``naive'' significance measure that sums up the weights of edges within communities. To avoid the trivial solution of assigning all nodes into one single community, for each community, we balance the total weights by a rescaling factor that penalizes its size. I.e., we choose the factor to be an increasing function of the community size. The criterion is therefore:

% \begin{equation}
%       R:=\sum_{k=1}^K \frac{1}{f(|C_k|)}\sum_{i, j\in C_k}A_{ij}w_{ij}
% \end{equation}
% where $K$ denotes the total number of communities. As mentioned in the last section we assume $K$ is known. For simplicity and flexibility, we choose $f$ to be the power function with a tuning parameter $\alpha$:
% \begin{equation}
%       f(t):=t^\alpha
% \end{equation}
% The criterion is then written as:
% \begin{equation}
%       R:=\sum_{k=1}^K \frac{1}{|C_k|^\alpha}\sum_{i, j\in C_k}A_{ij}w_{ij} \label{marginal_criterion}
% \end{equation}
% 
% Notice that (\ref{marginal_criterion}) is a family of stand alone community detection criteria on weighted networks. We discuss its properties while fixing edge weights $w_{ij}$ in the next section. First, we continue with modeling the edge weights $w_{ij}$'s as functions of node features.
% 
% We are now ready to propose the joint community detection criterion(JCDC). Summarizing the formulations in Sections 3.1 and 3.2, we optimize the following joint measure of community structure significance over all community assignments $C$ and coefficient $\bm{\beta}$:
% where $w$ is defined as in (\ref{weight_function}). The tuning parameters are $\alpha$ and $w_{\max}$ in $w$. In practice, to avoid extreme solutions of $\bm{\beta}$, we also impose a penalty on $\bm{\beta}$, as will be discussed in Section 4. The impact of the tuning parameters is analyzed in Section 4, and numerical experiments are presented in Section 6.

%\subsection{Determining edge weights}


%We now determine the weight function $w$. We start with describing generally desirable choices of $w$. First, in practice, different features on a node usually differ in their correlation to the underlying community structure thus in their relevance to our detection goal, and such differences are inherited by their induced similarities. Therefore, we choose $w$ to be a function of the linear combination of similarities on each node, i.e. $w(\bm{f_i}, \bm{f_j}; \bm{\beta}) = w(\langle \bm{\phi_{ij}},\bm{\beta} \rangle)$, where the coefficient $\bm{\beta}$  controls the impacts of different dimensions in $\bm{\phi_{ij}}$. In Section 4, we explain how the estimation of each dimension in $\bm{\beta}$ is connected to the learning of their correlation to the estimated community structure. \\

%The inner product, as the variable in function $w$, can be viewed as a comprehensive similarity measure that summarizes the similarities encoded in $\bm{\phi_{ij}}$. Recall that we assume that within communities, nodes display more similarities in their features. Therefore, $w$ is an increasing function of the comprehensive similarity $\langle \bm{\phi_{ij}},\bm{\beta} \rangle$. Notice that we do not restrict the signs of $\bm{\beta}$'s elements to the positive range, so as to preserve the flexibility to incorporate the so-called ``opposites attract'' features.\\

%Another desirable character of $w$ is concavity. Concavity guarantees the global uniqueness of the optimal $\bm{\beta}$. The detailed discussion on where the optimal $\bm{\beta}$ lies is in Section 4. A notable issue here is that mathematically, the combination of increasing $w$ and concavity unavoidably leads to possible negative weights on some edges, whose appearance depends on specific node feature values.  In our implementation, we truncate negative edge weights to $0$ while updating the community assignments $C$ with fixed edge weights, but do not restrict the edge weights to be positive when optimizing over $\bm{\beta}$. Empirically we discover that doing so improves both the precision and the robustness of the estimation result, as opposed to not truncating negative $w_{ij}$'s when updating $C$.\\
%\begin{enumerate}
%\item {\bf Exponential function:}

%where $w_{\max}$ is a tuning parameter greater than 1.
%\item {\bf Logit exponential function:}
%\begin{equation}
%w^{logit}(\bm{\phi_{ij}}, \bm{\beta}):=w_{\max}+\log\left( \frac{e^{\langle \bm{\phi_{ij}},\bm{\beta} \rangle}}{1+e^{\langle \bm{\phi_{ij}},\bm{\beta} \rangle}} \right)\label{weight_function2}
%\end{equation}
%\end{enumerate}
 %These two choices yield similar results in numerical experiments. Throughout this paper, we use the simpler exponential function, in numerical studies and applications.

%The approximated $\hat{\bm{\beta}}$ in (\ref{illustration_beta}) is bounded, due to ignoring higher order terms in the expansion of the exponential function. In reality, when the proportion of positive $\bm{\phi_{ij}}^{(z)}$'s increases above a certain threshold, the optimal $\bm{\beta}^{(z)}$ goes quickly to $+\infty$ as the proportion of positive $\bm{\phi_{ij}}^{(z)}$ goes to $1$. In the extreme case, $\phi_{ij}$'s within all communities that corresponds to $A_{ij}=1$ are positive, and the corresponding $\hat{\beta}$ is $\infty$. To remedy this issue, we introduce a penalty term in the criterion:
%\begin{align}
%%PL&:=\sum_k \frac{1}{|C_k|}\sum_{i, j\in C_k}(1-A_{ij})w_{ij}+\lambda\|\vec{\beta}\|\label{Pcriterion1}\\
%PR&:=\sum_k \frac{1}{|C_k|^\alpha}\sum_{i, j\in C_k}A_{ij}w(\bm{\phi_{ij}}; \bm{\beta})-\lambda\|\bm{\beta}\|_1\label{Pcriterion2}
%\end{align}

%Here we use the penalty term as a safeguard to avoid extreme solutions when optimizing $\bm{\beta}$ rather than using it to serve the purpose of variable selection. It is an independent question to study in further detail the shrinkage effects of different choices of $\lambda$. Notice that any positive $\lambda$ eliminates the possibility of infinite $\bm{\beta}$, since the first term in (\ref{Pcriterion2}) grows to $+\infty$ slower than linear. The choice of the tuning parameter $\lambda$ is a seperate topic for future studies. In practice, we found that choosing $\lambda=1$ works well for most artificial and real life networks that we experimented with. Choosing $\lambda>3$ usually eliminates all features and tends to be too sparse, based on empirical evidences on networks with varying configurations.


==> texsections/section_2__Yuan_Zhang____________2015-07-24_.tex <==
Our method is designed to look for the type of community structure, where nodes are more likely to connect to each other if they belong to the same community, thus communities tend to have more edges within themselves than between.  This is a very common intuitive definition of communities which is incorporated in many criteria used for community detection, for example, modularity \cite{NewmanPNAS}.   Our goal is to use such a community detection criterion based on the adjacency matrix alone, and add feature-based edge weights to improve detection.   Several criteria using the adjacency matrix alone are available, but having a simple criterion linear in the adjacency matrix makes optimization much more feasible in our particular situation, and we propose a new such criterion which turns out to work particularly well for our purposes.   Let $A$ denote the adjacency matrix with $A_{ij}=0$ if there is no edge between nodes $i$ and $j$,  and $A_{ij} > 0$ otherwise, which can be either 1 for unweighted networks or the edge weight for weighted networks.    The community detection criterion we start from is a very simple analogue of modularity, to be maximized over all possible label assignments $e$: 
\begin{equation}
      R(e)=\sum_{k=1}^K \frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k}A_{ij} \ . 
     \label{marginal_criterion}
\end{equation}
Here $e$ is the vector of node labels, with $e_i = k$ if node $i$ belongs to community $k$, for $k = 1, \dots, K$,  $\E_k = \{i: e_i = k\}$, and $|\E_k|$ is the number of nodes in community $k$.  We assume each node belongs to exactly one community, and the number of communities $K$ is fixed and known.  Rescaling by $|\E_k|^\alpha$ is designed to rule out trivial solutions that put all nodes in the same community, and $\alpha > 0$ is a tuning parameter.  When $\alpha=2$, the criterion is approximately the sum of edge densities within communities, and when $\alpha=1$, the criterion is the sum of average ``within community'' degrees, which both intuitively represent community structure.  
 This criterion can be shown to be consistent under the stochastic block model by checking the conditions of the general theorem in \cite{Bickel&Chen2009}.  

The ideal use of features with this criterion would be to use them to up-weigh edges within communities and down-weigh edges between them, thus enhancing the community structure in the observed network and making it easier to detect.  However, node features may not be perfectly correlated with community structure, different communities may be driven by different features, as pointed out by \cite{Jure_ego}, and features themselves may be noisy.  Thus we need to learn the impact of different features on communities as well as balance the roles of network information and the node features.   Let $f_i$ denote the $p$-dimensional feature vector of node $i$.   We propose a \emph{joint community detection criterion} (JCDC), 
\begin{equation}
	\max_{e, \beta} R(e, \beta; w_n):=\sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i,j\in \E_k}A_{ij}W(f_i, f_j, \beta_k; w_n) \label{JCDC}
\end{equation}
where $\alpha$ is a tuning parameter as in \eqref{marginal_criterion}, $\beta_k\in\mathbb{R}^p$ are the coefficient vectors that define the impact of each feature on different communities, and $\beta:=\{\beta_1,\ldots, \beta_K\}$.   Having a different $\beta_k$ for each community allows us to learn the roles different features may play in different communities.  The balance between the information from $A$ and $F:=\{f_1,\ldots,f_n\}$ is controlled by $w_n$, another tuning parameter which in general may depend on $n$. 

For the sake of simplicity, we model the edge weight $W(f_i, f_j, \beta_k; w_n)$ as a function of the node features $f_i$ and $f_j$ via a $p$-dimensional vector of their similarity measures $\phi_{ij} = \phi(f_i, f_j)$. The choice of similarity measures in $\phi$ depends on the type of $f_i$ (for example, on whether the features are numerical or categorical) and is determined on a case by case basis;  the only important property of similarity is that it assigns higher values to features that are more similar. To eliminate potential differences in units and scales, we standardize all $\phi_{ij}$ along each feature dimension.   Note that this trivially allows the inclusion of edge features  as well as node features, as long as they are converted to some sort of similarity.   Finally, the function $W$ should be increasing in $\langle \phi_{ij}, \beta \rangle$, which can be viewed as the ``overall similarity'' between nodes, and it is convenient to take $W$ to be concave to facilitate optimization.  Here we use the exponential function
\begin{equation}
w_{ijk} := W(f_i, f_j, \beta_k; w_n) = 
%W(\phi_{ij}, \beta_k; w_n) = 
w_n-e^{-\langle \phi_{ij},\beta_k \rangle}
\label{weight_function}
\end{equation}
One can use other functions of similar shapes, for example, the logit exponential function, which we found empirically to perform similarly.


==> texsections/section_33.tex <==
The joint community detection criterion needs to be optimized over both the community assignment $\bm{e}$ and the parameters  $\bm{\beta}$, which determine the edge weights $w_{ij}$.  Using block coordinate descent, we optimize the joint criterion by fixing one variable and optimizing over the other one, and iterating until convergence. 

\subsection{Optimizing over label assignments with fixed weights}
\label{sec:fixedbeta}
In this step we treat all edge weights $w_{ij}$'s as fixed constants. It is infeasible to search over all $n^K$ possible labels assignments, and, like\textcolor{cyan}{(similar to)} many other community detection methods, we rely on a greedy label switching algorithm to optimize over $\bm{e}$, specifically, the tabu search \cite{Glover:tabu}, which updates the label of one node at a time. When the target community sizes are large, our method allows for a simple local update which does not require recalculating the entire criterion.  For a node $i$,  the condition for the algorithm to prefer to assign it to community $k$ rather than $l$ is\textcolor{cyan}{[I corrected the formulation here. There should be ``+1'''s on two denominators]}, 
	\begin{align}
		\frac{S_{kk}+2S_{i\leftrightarrow k}}{|E_k+1|^\alpha} + \frac{S_{ll}}{|E_l|^\alpha}  & >  \frac{S_{kk}}{|E_k|^\alpha} + \frac{S_{ll}+2S_{i\leftrightarrow l}}{|E_l+1|^\alpha} \ ,  \label{k_vs_l_raw}
	\end{align}
where $S_{kk}$ and $S_{ll}$ denote twice the total edge weights in communities $k$ and $l$, respectively, and $S_{i\leftrightarrow k}$ and $S_{i\leftrightarrow k}$ denote the sum of edge weights between node $i$ and all \textcolor{cyan}{(other)} nodes in $E_k$ and $E_l$, respectively.  When $|E_k|$ and $|E_l|$ are large, \eqref{k_vs_l_raw} is approximately equivalent to 
	\begin{equation}
		\frac{S_{i \leftrightarrow k}}{|E_k|}\cdot \frac{|E_k|^{1-\alpha}}{|E_l|^{1-\alpha}} > \frac{S_{i \leftrightarrow l}}{|E_l|} \ .
\label{alpha_and_community_size}
	\end{equation}
The simplified condition \eqref{alpha_and_community_size} allows for a\textcolor{cyan}{[insert a space here]}``local'' update for the label of $i$ without calculating the entire criterion.  It also illustrates the impact of the tuning parameter $\alpha$:  when $\alpha=1$, both sides of \eqref{alpha_and_community_size} can be viewed as averaged weights of all edges connecting node $i$ to communities $E_k$ and $E_l$, respectively.  Then our method assigns node $i$ to the community with which it has the strongest connection.    When $\alpha \neq 1$, the LHS is multiplied by a factor $(|E_k|/|E_l|)^{1-\alpha}>1$.  Suppose $E_k$ is larger than $E_l$;  then choosing $0 < \alpha < 1$ increases the preference for assigning a node to the larger community, while  $\alpha>1$ favors smaller communities.

Note that all the $S$'s\textcolor{cyan}{($S$'es)} in \eqref{alpha_and_community_size} are functions of edge weights and thus depend on the tuning parameter $w_{\max}$. When $\bm{\beta}=\bm{0}$, all weights are equal to the constant $w_{\max}-1$.  On the other hand, for all values of $\bm{\beta}$ the sharp upper bound on any edge weight is $w_{\max}$. Therefore, the ratio $r_w =w_{\max}/(w_{\max}-1)$ is the maximum amount by which our method can  reweigh an edge. When $w_{\max}$ is large, $r_w\approx 1$, and thus the information from the network structure dominates. When $w_{\max}$ is close to $1$, $r_w$ is large and the feature-driven edge weights have a large  impact.  However,  even if $w_{\max}$ is close to 1, the features will not necessarily dominate the network information, especially in a sparse graph, since we only consider and reweigh observed edges.

While the tuning parameter $w_{\max}$ controls the amount of influence features can have on community detection, it does not affect the estimated parameters $\bm{\beta}$ for a fixed community assignment.  This is easy to see from rearranging terms in \eqref{JCDC}: 
\begin{equation}
	R(\bm{e}, \bm{\beta}) = \sum_{k=1}^K\frac{1}{|E_k|^\alpha}\sum_{(i, j)\in E_k}A_{ij}w_{\max} + \sum_{k=1}^K\frac{1}{|E_k|^\alpha}\sum_{(i, j)\in E_k}A_{ij}g(\bm{f}_i, \bm{f}_j; \bm{\beta}_k) \label{break_JCDC_to_two_terms}
\end{equation}
where $g(\cdot, \cdot ; \cdot):=w(\cdot, \cdot ; \cdot)-w_{\max}$. The tuning parameter $w_{\max}$ is only involved in the term that does not depend on $\bm{\beta}$.   

Asymptotically, if the feature weights satisfy some conditions, the optimal community assignment is consistent under the stochastic block model.  More precisely, let $\bm{c}$ be the true labels, and let $\rho_n P_{kl} = P(A_{ij = 1}| c_i = k \mbox{ and } c_j = l)$, where $\rho_n \rightarrow 0$ is the global edge probability scaling parameter.  Let $\tilde{P}_{kl}:=P_{kl}\mathbb{E}[w_{ij}|(i, j)\in (\bm{c}_k, \bm{c}_l)]$. If for any $a\neq b$, we have $\alpha(\tilde{P}_{aa}+\tilde{P}_{bb})>2\tilde{P}_{ab}$ for $\alpha\geq1$ and $(2^\alpha-1)\min(\tilde{P}_{aa},\tilde{P}_{bb})>\tilde{P}_{ab}$, then $\mathbb{P}(\hat{\bm{e}}=\bm{c})\to1$ if $n \rho_n /\log n\to+\infty$ and $\|\hat{\bm{e}}-\bm{c}\|\stackrel{p}{\to}0$ if $n \rho_n\to+\infty$. The proof follows the reasoning of \cite{Bickel&Chen2009} and \cite{Zhaoetal2012} and is omitted here due to length constraints.

\subsection{Optimizing over weights with fixed label assignments}

Since we chose a concave edge weight function \eqref{weight_function}, for a given community assignment $\bm{e}$ the joint criteiron is a concave function of $\bm{\beta}_k$, and it is straightforward to optimize over  $\bm{\beta}_k$ by gradient ascent.    The role of $\bm{\beta}_k$ is to control the impact of different features on each community.     One can show by a Taylor-series type expansion around the maximum (details omitted) and also observe empirically that for our method, the estimated $\hat{\bm{\beta}}_k$ is \textcolor{cyan}{(+positively)?} correlated with the feature similarity levels between nodes in community $k$.  Specifically, \textcolor{cyan}{(for the $d$th feature, $d\in\{1,\ldots,p\}$,)} we found that in practice the estimated $\hat{\bm{\beta}}_k^{(d)}$ is an increasing function of the sample mean of the corresponding similarity $\hat{\mathbb{E}}[\phi_{ij}|(i, j)\in E_k]$.    In other words, our method produces large estimated $\hat{\bm{\beta}}_k^{(d)}$'s for a feature $d$ if it has a high similarity value $\bm{\phi}_{ij}^{(d)}$'s in community $k$. However, in the extreme case, the optimal $\hat{\bm{\beta}}_{k}^{(d)}$ can be $+\infty$ if all $\bm{\phi}_{ij}^{(d)}$'s are positive in community $k$ or $-\infty$ if all $\bm{\phi}_{ij}^{(d)}$'s are negative.  To avoid extreme solutions like this\textcolor{cyan}{(such extreme solutions)}, we subtract a penalty term $\lambda\|\bm{\beta}\|$ from JCDC while optimizing over $\bm{\beta}$.    We use a small value of $\lambda$ that serves as a safeguard against extreme solutions and does not much affect moderate values of estimated $\bm{\beta}^{(d)}_k$.

In order to formally asses\textcolor{cyan}{(assess)} the significance of each feature for a particular community \textcolor{cyan}{(structure)}, we can perform a permutation test once we have \textcolor{cyan}{(the)} estimated $\bm{\beta}_k$ and the label assignments $\bm{e}$.  For each feature $d \in\{1,\ldots,p\}$, we generate a random permutation $(n_1, \ldots, n_N)$ of $(1, \ldots, N)$.  Then we permute the $d$th dimension of the node similarity measure $\bm{\phi}_{ij}^{(d)}$ into $\bm{\phi}_{n_i n_j}^{(d)}$ and optimize the joint community detection criterion over $\bm{\beta}^{(d)}$ while fixing all $\bm{\phi}_{ij}^{(d')}$ and $\bm{\beta}^{(d')}$ for $d'\neq d$. Repeating this many times gives us the null distribution for $\bm{\beta}^{(d)}$ under the hypothesis that the $d$-th feature has no impact on communities (since permuting the similarity values at random destroys any such relationship even if there was one).   This null distribution can be then used to compute a $p$-value for the estimated $\bm{\beta}_k^{(d)}$.   









% \section{Properties of the joint community detection criterion(JCDC)}
% 
% It is of interest to understand the community detection mechanism of the JCDC (\ref{JCDC}). We split the discussion into two parts: the analysis on maximizing (\ref{JCDC}) as a function of $C$ with fixed $\bm{\beta}$, and the analysis of the optimal $\bm{\beta}$ fixing $C$.

% \subsection{The JCDC as a community detection criterion on weighted networks}
% 
% In this subsection, we view JCDC as a function of $C$ fixing $\bm{\beta}$ and thus fixing all edge weights. We are interested in where the optimal $C$ lies, as well as its asymptotic properties under certain settings. We start with a few immediate observations on (\ref{JCDC}):
% 
% \begin{enumerate}
%       \item When $\alpha=2$, the criterion is approximately the sum of edge densities in each community.
%       \item When $\alpha=1$, the criterion is the sum of the average "within community" degree in each community. The "within community" degree for node $i\in C_k$ is the total number of edges between $i$ and other nodes in $C_k$.
%       \item When $\alpha=1$, maximizing $R$ is equivalent to minimizing the following rescaled loss:
% 	    \begin{equation}
% 		  L:=\sum_{k=1}^K \frac{1}{|C_k|}\sum_{i, j\in C_k}(1-A_{ij})
% 	    \end{equation}
% 	    which is a rescaled sum of the number of "structural holes" or missing edges, within each community, since $R+L\equiv N$. Notice the equivalence only holds under non-overlapping community scenario. The rescaled loss $L$ can be viewed as an extension of the criterion in the generalized K-means
% 	    \begin{equation}
% 		  \arg\min_C \sum_{k=1}^K \frac{1}{|C_k|}\sum_{i, j\in C_k}D(i, j)
% 	    \end{equation}
% 	    where $D(i, j)$ is a distance between $i$ and $j$, in this case a binary loss $(1-A_{ij})$. Note that the question here is whether we choose to trust the structural information provided by a sparse network $A$. If $A$ is too sparse, then the structural information provided by weighted $A$ may be highly noise, and the community extraction results based on weighted $A$ may be unstable. However, if the density of communities in $A$ is significant, but not comparable to the number of node pairs in the community, e.g. the number of edges in $C_k$ is in the order of $O(|C_k|)$.
% \end{enumerate}






%	\begin{equation}
%		\frac{S_{ik}}{|C_k|^\alpha} > \frac{S_{il}}{|C_l|^\alpha} \label{individual_update}
%	\end{equation}`
%The two sides in (\ref{individual_update}) can be viewed as rescaled measures of connectivity between the node $i$ and the two communities. When $\alpha=1$, both sides of Equation (\ref{individual_update}) have the interpretation of the averaged weights of parts between node $i$ and communities $C_k$ and $C_l$. Therefore, our method assigns each node $i$ to the community it is most tightly connected to.\\
%
%We now look at the impact of $\alpha$ on the eventual community detection outcome. Without loss of generality, we assume $|C_k|\geq |C_l|$. Rewritting (\ref{individual_update}) as:






% \subsection{Consistency of community detection under the Stochastic Blockmodel}
% 
% The formulation of (\ref{JCDC}), though not a direct extension of, matches the spirit of the Stochastic Blockmodel in the sense that they both regard the variance of edge densities in different parts of the network as mainly caused by the community assignments of the nodes involved. Therefore, we expect that our method produces asymptotically consistent community detection result under the block model. We state the consistency theorem below:\\
% 
% {\bf Theorem 1} Let all weights are the same, i.e., consider a binary network $A$. If for any community indices $a\neq b$, we have
% \begin{equation}
% \alpha(P_{aa}+P_{bb})>2P_{ab} \label{consistency}
% \end{equation}
% for $\alpha\geq 1$, or
% \begin{equation}
% (2^\alpha-1)\cdot\min(P_{aa}, P_{bb})>P_{ab}
% \end{equation}
% for $0<\alpha<1$, and the regularity conditions in \cite{Zhaoetal2012} are satisfied, then the JCDC (\ref{JCDC}) is strongly consistent when $\lambda_n/\log n\to+\infty$ and weakly consistent when $\lambda_n\to+\infty$ under the Stochastic Blockmodel as $n\to \infty$.\\
% 
% The proof is in the Appendix.\\
% 
% We clarify here that despite the fact that smaller $\alpha$ yields a stronger condition (\ref{consistency}), it does not mean a small $\alpha$ is worse than a large $\alpha$. First, currently there are no established theoretical results on convergence rates of any criterion under the Stochastic Blockmodel, or any other (more sophisticated) generative models. Second, the theorem states asymptotic properties, which may differ significantly for the networks with limited sizes.


%\subsection{The role of $w_{\max}$}\label{impact_of_wmax}

% the impact of the edge weights on the community detection results. Notice that both $\bm{\beta}$ and $w_{\max}$ control the magnitude of the influence of features on the community detection results, therefore it is important to clarify the differences in their roles. In our method, the node features influence the detection results via edge weights. The parameters $\bm{\beta}$ controls the influences of different features on the scalar edge weights $w_{ij}$'s, and $w_{\max}$ controls the impact of $w_{ij}$'s on the final detection results:
%\begin{center}
%\begin{minipage}[H, c]{0.4\textwidth} 
%\begin{tikzpicture}[->,>=stealth,shorten >=1pt, auto = center, node distance=3cm, 
%                    thick,data/.style={circle,draw,font=\sffamily\bfseries}, first para/.style={scale=0.7,draw,font=\sffamily\bfseries}, sec para/.style = {rectangle,scale=0.8, draw,dashed,font=\sffamily\Large\bfseries}] 
%\node[data] (fi) at (0, 4) {$\bm{f_i}$};
%\node[data] (fj) at (0, 2)  {$\bm{f_j}$};
%\node[data] (phiij) at (2, 3) {$\bm{\phi_{ij}}$};
%\node[data] (wij) at (4, 3) {$w_{ij}$};
%\node[data] (Aij) at (4, 1)  {$A_{ij}$};
%\node[data] (community) at (6, 2) {$C$};
%\node[data, draw=white] (beta) at (3,3.5) {$\bm{\beta}$};
%\node[data, draw=white] (wmax) at (5.2,3) {$w_{\max}$};
%\foreach \from/\to in {fi/phiij, fj/phiij, phiij/wij, wij/community, Aij/community} 
%    \draw (\from) -> (\to); 
%\end{tikzpicture}  
%\end{minipage}
%\end{center}

%The tuning parameter $w_{\max}$ comes from our specific formulation of the function of $w$, however, its role in the joint community detection framework has a universal meaning shared by any methodology that addresses the same problem. The philosophical question is on balancing the influence of the network $A$ and the features $\bm{f_i}$'s. When both $A$ and $F$ display community structures that are not necessarily in agreement with each other, we need to decide how much influence each of them has on the final community detection result when combining the two sources of data. Such balance cannot be learned automatically from data, and in practice it is chosen in a subjective and context dependent fashion. In Section 6, we show a simulation that illustrates the varying impact of node features on the final detection result under different choices of $w_{\max}$.

%Specifically, we consider the scalar case in which we only have one feature and this features is correlated to the community structure of community $k$, i.e. $\mathbb{E}[\phi_{ij}|(i, j)\in \bm{e}_k]>0$. The optimal $\bm{\beta}$ has no closed form solution, thus we implement an approximation to illustrate this point for small $\beta$ values. The second order Taylor expansion of $w$ gives:
%\begin{align}
%w_{ij}& = w_{\max} - e^{\phi_{ij}\beta_k}\\
%&\approx w_{\max}-1+\phi_{ij}\beta_k - (\phi_{ij}\beta_k)^2/2 \label{taylor_order2}
%\end{align}
%The corresponding (approximated) term in the joint criterion is therefore $\sum_{(i, j)\in\bm{e}_k}A_{ij}(2\phi_{ij}\beta_k - (\phi_{ij}\beta_k)^2)$ (ignoring the rescaling factor that does not affect $\hat{\beta}_k$), which gives
%\begin{align}
%\hat{\beta}_k &= \frac{\sum_{(i, j)\in\bm{e}_k}\phi_{ij}}{\sum_{(i, j)\in\bm{e}_k}\phi_{ij}^2} \to \frac{\mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]}{Var[\phi_{ij}|(i, j)\in\bm{e}_k] + \mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]^2} \label{increasing function}
%\end{align}
%which shows that $\hat{\beta}_k$ is an increasing function of $\mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]$ within a small neighborhood of 0, where the expansion (\ref{taylor_order2}) is a good approximation. As $\mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]$ grows larger such monotonicity still holds but need to be shown in numerical evaluations.
%The approximation (\ref{taylor_order2}) is precise when $\phi_{ij}\beta_k$'s are small, and (\ref{increasing function}) shows that for small $\$We can see that in the neighbor hood $\hat{\beta}_k$ is positive and increase with $\mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]$. When $\mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]$ grows larger, the approximation (\ref{taylor_order2}) is not precise and we need to numerically evaluate to see the positve association between $\hat{\beta}_k$ and $\mathbb{E}[\phi_{ij}|(i, j)\in\bm{e}_k]$.
%In practice, when the sample mean similarity within community $\hat{\mathbb{E}}[\phi_{ij}^{(z)}|(i, j)\in \bm{e}_k]$ is large, the corresponding $\hat{\bm{\beta}}^{(z)}$ is usually huge and dominating -- in the extreme case it is $\infty$ if all $\phi_{ij}^{(z)}$'s within the community have the same sign.


%The impact of $\bm{\beta}$, however, is restricted to the stage in which the edge weights are determined. It mainly serves the purpose of balancing the influence of different features. We will see later that in our method, features that are more correlated to the estimated community structure tend to have a larger estimated $\bm{\beta}$ coefficient. However, in practice, even the most correlated features may show significant differences in their clustering structure from that displayed in the network $A$, so the question of balancing the influences of $A$ and $F$ remains.\\

% \subsection{Interpretations of $\bm{\beta}$}
% 
% With the formulation of $w(\cdot)$ chosen, it is natural to ask what the optimal $\bm{\beta}$ means. Ideally, we expect to acquire a larger optimal $\bm{\beta}^{(z)}$ if the corresponding $z$th dimension $\bm{\phi}^{(z)}$ is closely correlated with the community structure, i.e., there is a significant difference between the $\bm{\phi}^{(z)}$ values within communities and between communities. This intuitive goal is the variable selection problem, an important practical aspect of all clustering methodology that makes use of multiple features or attributal information. Usually when people perform clustering techniques involving multiple features, it is of interest to know which dimensions in the features have essential connection to the clustering structure. The problem is relatively easier in supervised learning \cite{guoa2010modularized}, because the response in training data can be used to filter out irrelevant features. The problem is, however, much more difficult in unsupervised scenarios.\\
% 
% The joint community detection problem, for example, is a typical unsupervised learning problem. Specifically, in our approach the coefficient vector $\bm{\beta}$, which carries the information of the significance of node features, is learnt along with the community structure. This creates difficulty in even defining the concept of significance of node features. Notice that it is relatively easy to define the conditional significance, which means that we fix a community structure, and define the significant node feature dimensions to be those that are significantly correlated with the estimated community structure. Clearly, such significance definition depends on the community structure. It is unclear though how to or whether it is meaningful to define a gloable significance. Recall that our final goal is to optimize the joint community detection criterion over $C$ and $\bm{\beta}$ jointly, and currently the only feasible way is to optimize iteratively. Therefore, it is not unnatural that we base the feature selection and the related significance test on our best guess for the true underlying community structure, which is the estimated $C$.\\
% 
% In the discussion below, by "the community structure" we mean either the underground truth or a close guess. We aim at showing that our feature selection and testing methodology is effective in learning which dimensions are significantly correlated to the underlying community structure, if either we are in the oracle case and know the true community structure or have a close guess. One can view such feature selection and testing methodology as applied when the joint estimation is completed and mainly serves the interpretation of results. But the mechanism for this methodology - higher correlation with the estimated community structure yields larger estimated coefficient value - is consistent with our goal of joint community extraction. We optimize the joint community detection criterion iteratively, and throughout the procedure, we look for the possible agreement suggesting a certain community structure from both sources of information. Therefore, if a certain community assignment $C$ also separates certain dimension(s) of $\bm{\phi}$, this suggests that we found the desired agreement on two types of evidence.\\
% 
% As an illustration of the methodology, let us consider a specific choice of $w_{ij}$ as in (\ref{weight_function}):
% \begin{equation}
% w(\bm{\phi_{ij}}, \bm{\beta}):=w_{\max} - e^{-\langle \bm{\phi_{ij}}, \bm{\beta} \rangle} \label{specific_choice}
% \end{equation}
% To study the location of the optimal $\beta$, we take the second order approximation to the exponential function, i.e.
% \begin{equation}
% 	w(t)\approx w_{\max}-1+t-\frac{t^2}{2} 
% \end{equation}
% where we write $w$ as a function of a scalar variable since in (\ref{specific_choice}) $w$ is determined by the inner product of its two vector arguments. Plugging the approximation of $w$ into  JCDC (\ref{JCDC}) and ignoring the constants that do no involve $\bm{\beta}$, we have
% \begin{equation}
% 	R\approx\sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}\left( 2\bm{\beta}'\bm{\phi_{ij}} -  \bm{\beta}'(\bm{\phi_{ij}}\bm{\phi_{ij}}')\bm{\beta}\right)
% \end{equation}
% Therefore the optimal $\bm{\beta}$ is approximately:
% \begin{equation}
% 	\hat{\bm{\beta}} = \left( \sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}(\bm{\phi_{ij}}\bm{\phi_{ij}}') \right)^{-1}\cdot \left( \sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}\bm{\phi_{ij}} \right) \label{realized_version}
% \end{equation}
% 
% We simplify the problem by assuming that $A_{ij}$ is independent of $\bm{\phi_{ij}}$ given $C_k$, fixing the number of communities and assuming that as $n\to\infty$ the communities maintain the size ratios. We treat each $\bm{\phi_{ij}}$ as a realization of random variable $\bm{\phi}$. For further simplicity, we assume the dimensions of $\bm{\phi}$ to be identically distributed, having unit variance and equal covariance $\rho$ between each pair of different dimensions. We denote their common expectation by $u$. Therefore the population version($RHS_{pop}$) of the RHS in (\ref{realized_version}) is
% \begin{align}
% 	RHS_{pop} &= \left( (1-\rho)I + (\rho+u)\mathbbm{1}\mathbbm{1}' \right)^{-1}\cdot u\mathbbm{1}\\
% 			&= \frac{u Z}{1-\rho+(\rho+u) Z}\mathbbm{1}\label{illustration_beta}
% \end{align}
% where $Z$ is the dimension of $\bm{\phi}$. It is then straightforward to see that the population version of the optimal $\hat{\bm{\beta}}$, under the simplified case, is an increasing function of the total sum of $\mathbb{E}[\bm{\phi}]$ in each of their corresponding dimensions. Switching back to the realization, this means that for the $z$th feature, the more and larger positive $\phi_{ij}^{(z)}$ that we have within communities, the further $\hat{\bm{\theta}}^{(z)}$ departs from $0$ in the positive direction.\\


% \subsection{Penalty on $\bm{\beta}$}




%{\bf Iterative optimization procedure:}
%\begin{enumerate}
%\item Initialize $\hat{C}$ and set $\bm{\hat{\beta}}=\bm{0}$.
%\item Iterate until convergence
%	\begin{enumerate}
%	\item Fix $\bm{\hat{\beta}}$ and update $\hat{C}$
%		\begin{itemize}
%		\item Truncate negative edge weights to $0$.
%		\item Go through all nodes for multiple rounds. Within each round update each node's community assignment to the choice that maximizes the joint criterion
%		\end{itemize}
%	\item Fix $C$ and update $\bm{\hat{\beta}}$.
%	\end{enumerate}
%\item Perform the significance test on $\bm{\beta}$ based on $\hat{C}$.
%\end{enumerate}




==> texsections/section_3_BACKUP.tex <==
\section{Estimation}
\label{sec:optimization}
The joint community detection criterion needs to be optimized over both the community assignments $e$ and the feature parameters  $\beta$.   Using block coordinate descent, we optimize JCDC by alternately optimizing over the labels with fixed parameters and over the parameters with fixed labels, and iterating until convergence. 

\subsection{Optimizing over label assignments with fixed weights}
\label{sec:fixedbeta}
When parameters $\beta$ are fixed,  all edge weights $w_{ijk}$'s can be treated as known constants.  It is infeasible to search over all $n^K$ possible label assignments, and, like many other community detection methods, we rely on a greedy label switching algorithm to optimize over $e$, specifically, the tabu search \cite{Glover:tabu}, which updates the label of one node at a time.   Since our criterion involves the number of nodes in each community $|\E_k|$, no easy spectral approximations are available.   Fortunately, our method allows for a simple local approximate update which does not require recalculating the entire criterion.  For a given node $i$ considered for label switching, the algorithm will assign it to community $k$ rather than $l$ if  
	\begin{align}
		\frac{S_{kk}+2S_{i\leftrightarrow k}}{(|\E_k|+1)^\alpha} + \frac{S_{ll}}{|\E_l|^\alpha}  & >  \frac{S_{kk}}{|\E_k|^\alpha} + \frac{S_{ll}+2S_{i\leftrightarrow l}}{(|\E_l|+1)^\alpha} \ ,  \label{k_vs_l_raw}
	\end{align}
where $S_{kk}$ and $S_{ll}$ denote twice the total edge weights in communities $k$ and $l$, respectively, and $S_{i\leftrightarrow k}$ and $S_{i\leftrightarrow l}$ denote the sum of edge weights between node $i$ and all other nodes in $\E_k$ and $\E_l$, respectively.  When $|\E_k|$ and $|\E_l|$ are large, we can ignore $+1$ in the denominators, and \eqref{k_vs_l_raw} becomes 
\begin{equation}
		\frac{S_{i \leftrightarrow k}}{|\E_k|}\cdot \frac{|\E_k|^{1-\alpha}}{|\E_l|^{1-\alpha}} > \frac{S_{i \leftrightarrow l}}{|\E_l|} \ , 
\label{alpha_and_community_size}
\end{equation}
which allows for a ``local'' update for the label of node $i$ without calculating the entire criterion.  It also illustrates the impact of the tuning parameter $\alpha$:  when $\alpha=1$, the two sides of \eqref{alpha_and_community_size} can be viewed as averaged weights of all edges connecting node $i$ to communities $\E_k$ and $\E_l$, respectively.  Then our method assigns node $i$ to the community with which it has the strongest connection.    When $\alpha \neq 1$, the left hand side of \eqref{alpha_and_community_size} is multiplied by a factor $(|\E_k|/|\E_l|)^{1-\alpha}$.  Suppose $|\E_k|$ is larger than $|\E_l|$;  then choosing $0 < \alpha < 1$ indicates a preference for assigning a node to the larger community, while  $\alpha>1$ favors smaller communities.  A detailed numerical investigation of the role of $\alpha$ is provided in the Supplemental Material.   

Note that all the $S$'s in \eqref{alpha_and_community_size} are functions of edge weights and thus depend on the tuning parameter $w_n$. When $\beta=0$, all weights are equal to the constant $w_n-1$.  On the other hand, for all values of $\beta$ the sharp upper bound on any edge weight is $w_n$. Therefore, the ratio $w_n/(w_n-1)$ is the maximum amount by which our method can  reweigh an edge. When $w_n$ is large, $w_n/(w_n-1)\approx 1$, and thus the information from the network structure dominates. When $w_n$ is close to $1$, the ratio is large and the feature-driven edge weights have a large  impact.    See the Supplemental Material for more details on the choice of $w_n$.  

While the tuning parameter $w_n$ controls the amount of influence features can have on community detection, it does not affect the estimated parameters $\beta$ for a fixed community assignment.  This is easy to see from rearranging terms in \eqref{JCDC}: 
\begin{equation}
R(e, \beta; w_n) = \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k}A_{ij}w_n - \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} A_{ij} e^{-\langle \phi_{ij},\beta_k \rangle}
%g(\phi_{ij}; \beta_k) 
\label{break_JCDC_to_two_terms}
\end{equation}
%where $g(\phi_{ij} ; \beta_k):=w(\phi_{ij}; \beta_k)-w_n$. 
Note the tuning parameter $w_n$ is only involved in the term that does not depend on $\beta$.\\

\subsection{Optimizing over weights with fixed label assignments}

Since we chose a concave edge weight function \eqref{weight_function}, for a given community assignment $e$ the joint criterion is a concave function of $\beta_k$, and it is straightforward to optimize over  $\beta_k$ by gradient ascent.    The role of $\beta_k$ is to control the impact of different features on each community.     One can show by a Taylor-series type expansion around the maximum (details omitted) and also observe empirically that for our method, the estimated $\hat{\beta}_k$ is correlated with the feature similarity levels between nodes in community $k$.  Specifically, we found that in practice the estimated $\hat{\beta}_k^{(\ell)}$ is an increasing function of the sample mean of the corresponding similarity $\hat{\mathbb{E}}[\phi_{ij}^{(\ell)}|i, j\in \E_k]$, where $\hat{\beta}_k^{(\ell)}$ and $\phi_{ij}^{(\ell)}$ denote the elements of $\hat{\beta}_k$ and $\phi_{ij}$ corresponding to the $\ell$-th feature, $1\leq \ell \leq p$.    In other words, our method produces a large estimated $\hat{\beta}_k^{(\ell)}$ for a feature with high similarity values $\phi_{ij}^{(\ell)}$'s for $i, j \in \E_k$.  However, in the extreme case, the optimal $\hat{\beta}_{k}^{(\ell)}$ can be positive infinity if all $\phi_{ij}^{(\ell)}$'s are positive in community $k$ or negative infinity if all $\phi_{ij}^{(\ell)}$'s are negative.  To avoid extreme solutions like this, we subtract a penalty term $\lambda\|\beta\|_1$ from the criterion \eqref{JCDC} while optimizing over $\beta$.    We use a small value of $\lambda$ that serves as a safeguard against numerically unstable solutions and has little effect on other estimated $\beta^{(\ell)}_k$.  \tblue{For all numerical studies throughout this paper, we fix $\lambda$ at a small value $10^{-5}$.}

%To formally assess the significance of each feature for a particular community, we can perform a permutation test once we have estimated $\hat{\beta}_k$ and the label assignments $e$.  For each feature $\ell \in\{1,\ldots,p\}$ and each $k\in \{1,\ldots,K\}$, we generate a random permutation $(m_1,\ldots,m_n)$ of $(1, \ldots, n)$.  Then we permute the $\ell$-th dimension of the node similarity measure $\phi_{ij}^{(\ell)}$ into $\phi_{m_i m_j}^{(\ell)}$ and optimize the joint community detection criterion over $\beta_k^{(\ell)}$ while fixing all $\phi_{ij}^{(\ell')}$ for $\ell'\neq \ell$. Repeating this many times gives the null distribution for $\hat{\beta}_k^{(\ell)}$ under the hypothesis that the $\ell$-th feature has no impact on communities (since permuting the similarity values at random destroys any such impact).   This null distribution can be then used to compute a $p$-value for the estimated $\hat{\beta}_k^{(\ell)}$.   

\section{Consistency}
The proposed JCDC criterion \eqref{JCDC} is not model-based, but under certain models it is asymptotically consistent. We consider the setting where the network $A$ and the features $F$ are generated independently from a stochastic block model and a uniformly bounded distribution, respectively. Specifically, $\mathbb{P}(A_{ij}=1) = \rho_n P_{c_i c_j}$ where $\rho_n$ is a scaling factor controlling the overall edge density and $c = (c_1, \dots, c_n)$ are the true community labels.   Assume the following regularity conditions hold:
\begin{enumerate}
\item There exist global constants $M_\phi$ and $M_\beta$, such that $\|\phi_{ij}\|_2\leq M_\phi$ and $\|\beta_k\|_2\leq M_\beta$ for all $k$ (enforced in the feasible region of the optimization problem \eqref{JCDC}).    Assume the tuning parameter $w_n$ satisfies  $\log w_n> M_\phi M_\beta$. \label{condition_1}
\item Let ${\cal C}_k:=\{i: c_i = k\}$. There exists a global constant $\pi_0$ such that $|C_k|\geq \pi_0 n > 0$. \label{condition_2}
\item  For all $1\leq k<l \leq K$,  $2(K-1)P_{kl}<\min(P_{kk}, P_{ll})$. \label{condition_3}
\end{enumerate}

Condition \ref{condition_1} states that node feature similarities are uniformly bounded.  This is a mild condition in many applications as the node features are often themselves uniformly bounded. In practice, for numerical stability the user may normalize node features and discard individual features with very low variance, before calculating the corresponding similarities $\phi$. Condition \ref{condition_2} guarantees communities do not vanish asymptotically.   %Condition \ref{condition_3} guarantees the within-community probabilities of edges are sufficiently large compared to between-community probabilities.  

\begin{theorem}[Consistency of JCDC] Under conditions \ref{condition_1}, \ref{condition_2}  and \ref{condition_3}, 
if $n\rho_n\to\infty$, $w_n \rho_n\to \infty$, and the parameter $\alpha$ satisfies 
\begin{equation}
\frac{\max_{k, l}2(K-1)P_{kl}}{\min_{k,l}(P_{kk}, P_{ll})}<\alpha\leq 1 %\label{condition_3}
\end{equation}
then we have, for any fixed $\delta>0$, 
\begin{equation}
\mathbb{P}\left( \|\arg\max_{e}(\max_{\beta} R(e,\beta;w_n)) - c\|_1/n > \delta \right) \to 0 \ . 
\end{equation}
\end{theorem}
The proof of the theorem is given in the Supplemental Material.

% \section{Properties of the joint community detection criterion(JCDC)}
% 
% It is of interest to understand the community detection mechanism of the JCDC (\ref{JCDC}). We split the discussion into two parts: the analysis on maximizing (\ref{JCDC}) as a function of $C$ with fixed $\beta$, and the analysis of the optimal $\beta$ fixing $C$.

% \subsection{The JCDC as a community detection criterion on weighted networks}
% 
% In this subsection, we view JCDC as a function of $C$ fixing $\beta$ and thus fixing all edge weights. We are interested in where the optimal $C$ lies, as well as its asymptotic properties under certain settings. We start with a few immediate observations on (\ref{JCDC}):
% 
% \begin{enumerate}
%       \item When $\alpha=2$, the criterion is approximately the sum of edge densities in each community.
%       \item When $\alpha=1$, the criterion is the sum of the average "within community" degree in each community. The "within community" degree for node $i\in C_k$ is the total number of edges between $i$ and other nodes in $C_k$.
%       \item When $\alpha=1$, maximizing $R$ is equivalent to minimizing the following rescaled loss:
% 	    \begin{equation}
% 		  L:=\sum_{k=1}^K \frac{1}{|C_k|}\sum_{i, j\in C_k}(1-A_{ij})
% 	    \end{equation}
% 	    which is a rescaled sum of the number of "structural holes" or missing edges, within each community, since $R+L\equiv N$. Notice the equivalence only holds under non-overlapping community scenario. The rescaled loss $L$ can be viewed as an extension of the criterion in the generalized K-means
% 	    \begin{equation}
% 		  \arg\min_C \sum_{k=1}^K \frac{1}{|C_k|}\sum_{i, j\in C_k}D(i, j)
% 	    \end{equation}
% 	    where $D(i, j)$ is a distance between $i$ and $j$, in this case a binary loss $(1-A_{ij})$. Note that the question here is whether we choose to trust the structural information provided by a sparse network $A$. If $A$ is too sparse, then the structural information provided by weighted $A$ may be highly noise, and the community extraction results based on weighted $A$ may be unstable. However, if the density of communities in $A$ is significant, but not comparable to the number of node pairs in the community, e.g. the number of edges in $C_k$ is in the order of $O(|C_k|)$.
% \end{enumerate}






%	\begin{equation}
%		\frac{S_{ik}}{|C_k|^\alpha} > \frac{S_{il}}{|C_l|^\alpha} \label{individual_update}
%	\end{equation}`
%The two sides in (\ref{individual_update}) can be viewed as rescaled measures of connectivity between the node $i$ and the two communities. When $\alpha=1$, both sides of Equation (\ref{individual_update}) have the interpretation of the averaged weights of parts between node $i$ and communities $C_k$ and $C_l$. Therefore, our method assigns each node $i$ to the community it is most tightly connected to.\\
%
%We now look at the impact of $\alpha$ on the eventual community detection outcome. Without loss of generality, we assume $|C_k|\geq |C_l|$. Rewriting (\ref{individual_update}) as:






% \subsection{Consistency of community detection under the Stochastic Blockmodel}
% 
% The formulation of (\ref{JCDC}), though not a direct extension of, matches the spirit of the Stochastic Blockmodel in the sense that they both regard the variance of edge densities in different parts of the network as mainly caused by the community assignments of the nodes involved. Therefore, we expect that our method produces asymptotically consistent community detection result under the block model. We state the consistency theorem below:\\
% 
% {\bf Theorem 1} Let all weights are the same, i.e., consider a binary network $A$. If for any community indices $a\neq b$, we have
% \begin{equation}
% \alpha(P_{aa}+P_{bb})>2P_{ab} \label{consistency}
% \end{equation}
% for $\alpha\geq 1$, or
% \begin{equation}
% (2^\alpha-1)\cdot\min(P_{aa}, P_{bb})>P_{ab}
% \end{equation}
% for $0<\alpha<1$, and the regularity conditions in \cite{Zhaoetal2012} are satisfied, then the JCDC (\ref{JCDC}) is strongly consistent when $\lambda_n/\log n\to+\infty$ and weakly consistent when $\lambda_n\to+\infty$ under the Stochastic Blockmodel as $n\to \infty$.\\
% 
% The proof is in the Appendix.\\
% 
% We clarify here that despite the fact that smaller $\alpha$ yields a stronger condition (\ref{consistency}), it does not mean a small $\alpha$ is worse than a large $\alpha$. First, currently there are no established theoretical results on convergence rates of any criterion under the Stochastic Blockmodel, or any other (more sophisticated) generative models. Second, the theorem states asymptotic properties, which may differ significantly for the networks with limited sizes.


%\subsection{The role of $w_{\max}$}\label{impact_of_wmax}

% the impact of the edge weights on the community detection results. Notice that both $\beta$ and $w_{\max}$ control the magnitude of the influence of features on the community detection results, therefore it is important to clarify the differences in their roles. In our method, the node features influence the detection results via edge weights. The parameters $\beta$ controls the influences of different features on the scalar edge weights $w_{ij}$'s, and $w_{\max}$ controls the impact of $w_{ij}$'s on the final detection results:
%\begin{center}
%\begin{minipage}[H, c]{0.4\textwidth} 
%\begin{tikzpicture}[->,>=stealth,shorten >=1pt, auto = center, node distance=3cm, 
%                    thick,data/.style={circle,draw,font=\sffamily\bfseries}, first para/.style={scale=0.7,draw,font=\sffamily\bfseries}, sec para/.style = {rectangle,scale=0.8, draw,dashed,font=\sffamily\Large\bfseries}] 
%\node[data] (fi) at (0, 4) {$\bm{f_i}$};
%\node[data] (fj) at (0, 2)  {$\bm{f_j}$};
%\node[data] (phiij) at (2, 3) {$\bm{\phi_{ij}}$};
%\node[data] (wij) at (4, 3) {$w_{ij}$};
%\node[data] (Aij) at (4, 1)  {$A_{ij}$};
%\node[data] (community) at (6, 2) {$C$};
%\node[data, draw=white] (beta) at (3,3.5) {$\beta$};
%\node[data, draw=white] (wmax) at (5.2,3) {$w_{\max}$};
%\foreach \from/\to in {fi/phiij, fj/phiij, phiij/wij, wij/community, Aij/community} 
%    \draw (\from) -> (\to); 
%\end{tikzpicture}  
%\end{minipage}
%\end{center}

%The tuning parameter $w_{\max}$ comes from our specific formulation of the function of $w$, however, its role in the joint community detection framework has a universal meaning shared by any methodology that addresses the same problem. The philosophical question is on balancing the influence of the network $A$ and the features $\bm{f_i}$'s. When both $A$ and $F$ display community structures that are not necessarily in agreement with each other, we need to decide how much influence each of them has on the final community detection result when combining the two sources of data. Such balance cannot be learned automatically from data, and in practice it is chosen in a subjective and context dependent fashion. In Section 6, we show a simulation that illustrates the varying impact of node features on the final detection result under different choices of $w_{\max}$.

%Specifically, we consider the scalar case in which we only have one feature and this features is correlated to the community structure of community $k$, i.e. $\mathbb{E}[\phi_{ij}|(i, j)\in e_k]>0$. The optimal $\beta$ has no closed form solution, thus we implement an approximation to illustrate this point for small $\beta$ values. The second order Taylor expansion of $w$ gives:
%\begin{align}
%w_{ij}& = w_{\max} - e^{\phi_{ij}\beta_k}\\
%&\approx w_{\max}-1+\phi_{ij}\beta_k - (\phi_{ij}\beta_k)^2/2 \label{taylor_order2}
%\end{align}
%The corresponding (approximated) term in JCDC is therefore $\sum_{(i, j)\ine_k}A_{ij}(2\phi_{ij}\beta_k - (\phi_{ij}\beta_k)^2)$ (ignoring the rescaling factor that does not affect $\hat{\beta}_k$), which gives
%\begin{align}
%\hat{\beta}_k &= \frac{\sum_{(i, j)\ine_k}\phi_{ij}}{\sum_{(i, j)\ine_k}\phi_{ij}^2} \to \frac{\mathbb{E}[\phi_{ij}|(i, j)\ine_k]}{Var[\phi_{ij}|(i, j)\ine_k] + \mathbb{E}[\phi_{ij}|(i, j)\ine_k]^2} \label{increasing function}
%\end{align}
%which shows that $\hat{\beta}_k$ is an increasing function of $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$ within a small neighborhood of 0, where the expansion (\ref{taylor_order2}) is a good approximation. As $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$ grows larger such monotonicity still holds but need to be shown in numerical evaluations.
%The approximation (\ref{taylor_order2}) is precise when $\phi_{ij}\beta_k$'s are small, and (\ref{increasing function}) shows that for small $\$We can see that in the neighbor hood $\hat{\beta}_k$ is positive and increase with $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$. When $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$ grows larger, the approximation (\ref{taylor_order2}) is not precise and we need to numerically evaluate to see the positive association between $\hat{\beta}_k$ and $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$.
%In practice, when the sample mean similarity within community $\hat{\mathbb{E}}[\phi_{ij}^{(z)}|(i, j)\in e_k]$ is large, the corresponding $\hat{\beta}^{(z)}$ is usually huge and dominating -- in the extreme case it is $\infty$ if all $\phi_{ij}^{(z)}$'s within the community have the same sign.


%The impact of $\beta$, however, is restricted to the stage in which the edge weights are determined. It mainly serves the purpose of balancing the influence of different features. We will see later that in our method, features that are more correlated to the estimated community structure tend to have a larger estimated $\beta$ coefficient. However, in practice, even the most correlated features may show significant differences in their clustering structure from that displayed in the network $A$, so the question of balancing the influences of $A$ and $F$ remains.\\

% \subsection{Interpretations of $\beta$}
% 
% With the formulation of $w(\cdot)$ chosen, it is natural to ask what the optimal $\beta$ means. Ideally, we expect to acquire a larger optimal $\beta^{(z)}$ if the corresponding $z$-th dimension $\phi^{(z)}$ is closely correlated with the community structure, i.e., there is a significant difference between the $\phi^{(z)}$ values within communities and between communities. This intuitive goal is the variable selection problem, an important practical aspect of all clustering methodology that makes use of multiple features or attribute information. Usually when people perform clustering techniques involving multiple features, it is of interest to know which dimensions in the features have essential connection to the clustering structure. The problem is relatively easier in supervised learning \cite{guoa2010modularized}, because the response in training data can be used to filter out irrelevant features. The problem is, however, much more difficult in unsupervised scenarios.\\
% 
% The joint community detection problem, for example, is a typical unsupervised learning problem. Specifically, in our approach the coefficient vector $\beta$, which carries the information of the significance of node features, is learnt along with the community structure. This creates difficulty in even defining the concept of significance of node features. Notice that it is relatively easy to define the conditional significance, which means that we fix a community structure, and define the significant node feature dimensions to be those that are significantly correlated with the estimated community structure. Clearly, such significance definition depends on the community structure. It is unclear though how to or whether it is meaningful to define a global significance. Recall that our final goal is to optimize the joint community detection criterion over $C$ and $\beta$ jointly, and currently the only feasible way is to optimize iteratively. Therefore, it is not unnatural that we base the feature selection and the related significance test on our best guess for the true underlying community structure, which is the estimated $C$.\\
% 
% In the discussion below, by "the community structure" we mean either the underground truth or a close guess. We aim at showing that our feature selection and testing methodology is effective in learning which dimensions are significantly correlated to the underlying community structure, if either we are in the oracle case and know the true community structure or have a close guess. One can view such feature selection and testing methodology as applied when the joint estimation is completed and mainly serves the interpretation of results. But the mechanism for this methodology - higher correlation with the estimated community structure yields larger estimated coefficient value - is consistent with our goal of joint community extraction. We optimize the joint community detection criterion iteratively, and throughout the procedure, we look for the possible agreement suggesting a certain community structure from both sources of information. Therefore, if a certain community assignment $C$ also separates certain dimension(s) of $\phi$, this suggests that we found the desired agreement on two types of evidence.\\
% 
% As an illustration of the methodology, let us consider a specific choice of $w_{ij}$ as in (\ref{weight_function}):
% \begin{equation}
% w(\bm{\phi_{ij}}, \beta):=w_{\max} - e^{-\langle \bm{\phi_{ij}}, \beta \rangle} \label{specific_choice}
% \end{equation}
% To study the location of the optimal $\beta$, we take the second order approximation to the exponential function, i.e.
% \begin{equation}
% 	w(t)\approx w_{\max}-1+t-\frac{t^2}{2} 
% \end{equation}
% where we write $w$ as a function of a scalar variable since in (\ref{specific_choice}) $w$ is determined by the inner product of its two vector arguments. Plugging the approximation of $w$ into  JCDC (\ref{JCDC}) and ignoring the constants that do no involve $\beta$, we have
% \begin{equation}
% 	R\approx\sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}\left( 2\beta'\bm{\phi_{ij}} -  \beta'(\bm{\phi_{ij}}\bm{\phi_{ij}}')\beta\right)
% \end{equation}
% Therefore the optimal $\beta$ is approximately:
% \begin{equation}
% 	\hat{\beta} = \left( \sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}(\bm{\phi_{ij}}\bm{\phi_{ij}}') \right)^{-1}\cdot \left( \sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}\bm{\phi_{ij}} \right) \label{realized_version}
% \end{equation}
% 
% We simplify the problem by assuming that $A_{ij}$ is independent of $\bm{\phi_{ij}}$ given $C_k$, fixing the number of communities and assuming that as $n\to\infty$ the communities maintain the size ratios. We treat each $\bm{\phi_{ij}}$ as a realization of random variable $\phi$. For further simplicity, we assume the dimensions of $\phi$ to be identically distributed, having unit variance and equal covariance $\rho$ between each pair of different dimensions. We denote their common expectation by $u$. Therefore the population version($RHS_{pop}$) of the RHS in (\ref{realized_version}) is
% \begin{align}
% 	RHS_{pop} &= \left( (1-\rho)I + (\rho+u)\mathbbm{1}\mathbbm{1}' \right)^{-1}\cdot u\mathbbm{1}\\
% 			&= \frac{u Z}{1-\rho+(\rho+u) Z}\mathbbm{1}\label{illustration_beta}
% \end{align}
% where $Z$ is the dimension of $\phi$. It is then straightforward to see that the population version of the optimal $\hat{\beta}$, under the simplified case, is an increasing function of the total sum of $\mathbb{E}[\phi]$ in each of their corresponding dimensions. Switching back to the realization, this means that for the $z$-th feature, the more and larger positive $\phi_{ij}^{(z)}$ that we have within communities, the further $\hat{\bm{\theta}}^{(z)}$ departs from $0$ in the positive direction.\\


% \subsection{Penalty on $\beta$}




%{\bf Iterative optimization procedure:}
%\begin{enumerate}
%\item Initialize $\hat{C}$ and set $\bm{\hat{\beta}}=0$.
%\item Iterate until convergence
%	\begin{enumerate}
%	\item Fix $\bm{\hat{\beta}}$ and update $\hat{C}$
%		\begin{itemize}
%		\item Truncate negative edge weights to $0$.
%		\item Go through all nodes for multiple rounds. Within each round update each node's community assignment to the choice that maximizes JCDC
%		\end{itemize}
%	\item Fix $C$ and update $\bm{\hat{\beta}}$.
%	\end{enumerate}
%\item Perform the significance test on $\beta$ based on $\hat{C}$.
%\end{enumerate}




==> texsections/section_3__Yuan_Zhang____________2015-07-24_.tex <==
\section{Estimation}
\label{sec:optimization}
The joint community detection criterion needs to be optimized over both the community assignments $e$ and the feature parameters  $\beta$.   Using block coordinate descent, we optimize JCDC by alternately optimizing over the labels with fixed parameters and over the parameters with fixed labels, and iterating until convergence. 

\subsection{Optimizing over label assignments with fixed weights}
\label{sec:fixedbeta}
When parameters $\beta$ are fixed,  all edge weights $w_{ijk}$'s can be treated as known constants.  It is infeasible to search over all $n^K$ possible label assignments, and, like many other community detection methods, we rely on a greedy label switching algorithm to optimize over $e$, specifically, the tabu search \cite{Glover:tabu}, which updates the label of one node at a time.   Since our criterion involves the number of nodes in each community $|\E_k|$, no easy spectral approximations are available.   Fortunately, our method allows for a simple local approximate update which does not require recalculating the entire criterion.  For a given node $i$ considered for label switching, the algorithm will assign it to community $k$ rather than $l$ if  
	\begin{align}
		\frac{S_{kk}+2S_{i\leftrightarrow k}}{(|\E_k|+1)^\alpha} + \frac{S_{ll}}{|\E_l|^\alpha}  & >  \frac{S_{kk}}{|\E_k|^\alpha} + \frac{S_{ll}+2S_{i\leftrightarrow l}}{(|\E_l|+1)^\alpha} \ ,  \label{k_vs_l_raw}
	\end{align}
where $S_{kk}$ and $S_{ll}$ denote twice the total edge weights in communities $k$ and $l$, respectively, and $S_{i\leftrightarrow k}$ and $S_{i\leftrightarrow l}$ denote the sum of edge weights between node $i$ and all other nodes in $\E_k$ and $\E_l$, respectively.  When $|\E_k|$ and $|\E_l|$ are large, we can ignore $+1$ in the denominators, and \eqref{k_vs_l_raw} becomes 
\begin{equation}
		\frac{S_{i \leftrightarrow k}}{|\E_k|}\cdot \frac{|\E_k|^{1-\alpha}}{|\E_l|^{1-\alpha}} > \frac{S_{i \leftrightarrow l}}{|\E_l|} \ , 
\label{alpha_and_community_size}
\end{equation}
which allows for a ``local'' update for the label of node $i$ without calculating the entire criterion.  It also illustrates the impact of the tuning parameter $\alpha$:  when $\alpha=1$, the two sides of \eqref{alpha_and_community_size} can be viewed as averaged weights of all edges connecting node $i$ to communities $\E_k$ and $\E_l$, respectively.  Then our method assigns node $i$ to the community with which it has the strongest connection.    When $\alpha \neq 1$, the left hand side of \eqref{alpha_and_community_size} is multiplied by a factor $(|\E_k|/|\E_l|)^{1-\alpha}$.  Suppose $|\E_k|$ is larger than $|\E_l|$;  then choosing $0 < \alpha < 1$ indicates a preference for assigning a node to the larger community, while  $\alpha>1$ favors smaller communities.  A detailed numerical investigation of the role of $\alpha$ is provided in the Supplemental Material.   

Note that all the $S$'s in \eqref{alpha_and_community_size} are functions of edge weights and thus depend on the tuning parameter $w_n$. When $\beta=0$, all weights are equal to the constant $w_n-1$.  On the other hand, for all values of $\beta$ the sharp upper bound on any edge weight is $w_n$. Therefore, the ratio $w_n/(w_n-1)$ is the maximum amount by which our method can  reweigh an edge. When $w_n$ is large, $w_n/(w_n-1)\approx 1$, and thus the information from the network structure dominates. When $w_n$ is close to $1$, the ratio is large and the feature-driven edge weights have a large  impact.    See the Supplemental Material for more details on the choice of $w_n$.  

While the tuning parameter $w_n$ controls the amount of influence features can have on community detection, it does not affect the estimated parameters $\beta$ for a fixed community assignment.  This is easy to see from rearranging terms in \eqref{JCDC}: 
\begin{equation}
R(e, \beta; w_n) = \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k}A_{ij}w_n - \sum_{k=1}^K\frac{1}{|\E_k|^\alpha}\sum_{i, j\in \E_k} A_{ij} e^{-\langle \phi_{ij},\beta_k \rangle}
%g(\phi_{ij}; \beta_k) 
\label{break_JCDC_to_two_terms}
\end{equation}
%where $g(\phi_{ij} ; \beta_k):=w(\phi_{ij}; \beta_k)-w_n$. 
Note the tuning parameter $w_n$ is only involved in the term that does not depend on $\beta$.\\

\subsection{Optimizing over weights with fixed label assignments}

Since we chose a concave edge weight function \eqref{weight_function}, for a given community assignment $e$ the joint criterion is a concave function of $\beta_k$, and it is straightforward to optimize over  $\beta_k$ by gradient ascent.    The role of $\beta_k$ is to control the impact of different features on each community.     One can show by a Taylor-series type expansion around the maximum (details omitted) and also observe empirically that for our method, the estimated $\hat{\beta}_k$ is correlated with the feature similarity levels between nodes in community $k$.  Specifically, we found that in practice the estimated $\hat{\beta}_k^{(\ell)}$ is an increasing function of the sample mean of the corresponding similarity $\hat{\mathbb{E}}[\phi_{ij}^{(\ell)}|i, j\in \E_k]$, where $\hat{\beta}_k^{(\ell)}$ and $\phi_{ij}^{(\ell)}$ denote the elements of $\hat{\beta}_k$ and $\phi_{ij}$ corresponding to the $\ell$-th feature, $1\leq \ell \leq p$.    In other words, our method produces a large estimated $\hat{\beta}_k^{(\ell)}$ for a feature with high similarity values $\phi_{ij}^{(\ell)}$'s for $i, j \in \E_k$.  However, in the extreme case, the optimal $\hat{\beta}_{k}^{(\ell)}$ can be positive infinity if all $\phi_{ij}^{(\ell)}$'s are positive in community $k$ or negative infinity if all $\phi_{ij}^{(\ell)}$'s are negative.  To avoid extreme solutions like this, we subtract a penalty term $\lambda\|\beta\|_1$ from the criterion \eqref{JCDC} while optimizing over $\beta$.    We use a small value of $\lambda$ that serves as a safeguard against numerically unstable solutions and has little effect on other estimated $\beta^{(\ell)}_k$.  \tblue{For all numerical studies throughout this paper, we fix $\lambda$ at $10^{-5}$, which, empirically, has negligible impact on estimations.}

%To formally assess the significance of each feature for a particular community, we can perform a permutation test once we have estimated $\hat{\beta}_k$ and the label assignments $e$.  For each feature $\ell \in\{1,\ldots,p\}$ and each $k\in \{1,\ldots,K\}$, we generate a random permutation $(m_1,\ldots,m_n)$ of $(1, \ldots, n)$.  Then we permute the $\ell$-th dimension of the node similarity measure $\phi_{ij}^{(\ell)}$ into $\phi_{m_i m_j}^{(\ell)}$ and optimize the joint community detection criterion over $\beta_k^{(\ell)}$ while fixing all $\phi_{ij}^{(\ell')}$ for $\ell'\neq \ell$. Repeating this many times gives the null distribution for $\hat{\beta}_k^{(\ell)}$ under the hypothesis that the $\ell$-th feature has no impact on communities (since permuting the similarity values at random destroys any such impact).   This null distribution can be then used to compute a $p$-value for the estimated $\hat{\beta}_k^{(\ell)}$.   

\section{Consistency}
The proposed JCDC criterion \eqref{JCDC} is not model-based, but under certain models it is asymptotically consistent. We consider the setting where the network $A$ and the features $F$ are generated independently from a stochastic block model and a uniformly bounded distribution, respectively. Specifically, $\mathbb{P}(A_{ij}=1) = \rho_n P_{c_i c_j}$ where $\rho_n$ is a scaling factor controlling the overall edge density and $c = (c_1, \dots, c_n)$ are the true community labels.   Assume the following regularity conditions hold:
\begin{enumerate}
\item There exist global constants $M_\phi$ and $M_\beta$, such that $\|\phi_{ij}\|_2\leq M_\phi$ and $\|\beta_k\|_2\leq M_\beta$ for all $k$ (enforced in the feasible region of the optimization problem \eqref{JCDC}).    Assume the tuning parameter $w_n$ satisfies  $\log w_n> M_\phi M_\beta$. \label{condition_1}
\item Let ${\cal C}_k:=\{i: c_i = k\}$. There exists a global constant $\pi_0$ such that $|C_k|\geq \pi_0 n > 0$ (also enforced in the optimization \eqref{JCDC}). \label{condition_2}
\item  For all $1\leq k<l \leq K$,  $2(K-1)P_{kl}<\min(P_{kk}, P_{ll})$. \label{condition_3}
\end{enumerate}

Condition \ref{condition_1} states that node feature similarities are uniformly bounded.  This is a mild condition in many applications as the node features are often themselves uniformly bounded. In practice, for numerical stability the user may normalize node features and discard individual features with very low variance, before calculating the corresponding similarities $\phi$. Condition \ref{condition_2} guarantees communities do not vanish asymptotically.   %Condition \ref{condition_3} guarantees the within-community probabilities of edges are sufficiently large compared to between-community probabilities.  

\begin{theorem}[Consistency of JCDC] Under conditions \ref{condition_1}, \ref{condition_2}  and \ref{condition_3}, 
if $n\rho_n\to\infty$, $w_n \rho_n\to \infty$, and the parameter $\alpha$ satisfies 
\begin{equation}
\frac{\max_{k, l}2(K-1)P_{kl}}{\min_{k,l}(P_{kk}, P_{ll})}<\alpha\leq 1 %\label{condition_3}
\end{equation}
then we have, for any fixed $\delta>0$, 
\begin{equation}
\mathbb{P}\left( \|\arg\max_{e}(\max_{\beta} R(e,\beta;w_n)) - c\|_1/n > \delta \right) \to 0 \ . 
\end{equation}
\end{theorem}
The proof of the theorem is given in the Supplemental Material.

% \section{Properties of the joint community detection criterion(JCDC)}
% 
% It is of interest to understand the community detection mechanism of the JCDC (\ref{JCDC}). We split the discussion into two parts: the analysis on maximizing (\ref{JCDC}) as a function of $C$ with fixed $\beta$, and the analysis of the optimal $\beta$ fixing $C$.

% \subsection{The JCDC as a community detection criterion on weighted networks}
% 
% In this subsection, we view JCDC as a function of $C$ fixing $\beta$ and thus fixing all edge weights. We are interested in where the optimal $C$ lies, as well as its asymptotic properties under certain settings. We start with a few immediate observations on (\ref{JCDC}):
% 
% \begin{enumerate}
%       \item When $\alpha=2$, the criterion is approximately the sum of edge densities in each community.
%       \item When $\alpha=1$, the criterion is the sum of the average "within community" degree in each community. The "within community" degree for node $i\in C_k$ is the total number of edges between $i$ and other nodes in $C_k$.
%       \item When $\alpha=1$, maximizing $R$ is equivalent to minimizing the following rescaled loss:
% 	    \begin{equation}
% 		  L:=\sum_{k=1}^K \frac{1}{|C_k|}\sum_{i, j\in C_k}(1-A_{ij})
% 	    \end{equation}
% 	    which is a rescaled sum of the number of "structural holes" or missing edges, within each community, since $R+L\equiv N$. Notice the equivalence only holds under non-overlapping community scenario. The rescaled loss $L$ can be viewed as an extension of the criterion in the generalized K-means
% 	    \begin{equation}
% 		  \arg\min_C \sum_{k=1}^K \frac{1}{|C_k|}\sum_{i, j\in C_k}D(i, j)
% 	    \end{equation}
% 	    where $D(i, j)$ is a distance between $i$ and $j$, in this case a binary loss $(1-A_{ij})$. Note that the question here is whether we choose to trust the structural information provided by a sparse network $A$. If $A$ is too sparse, then the structural information provided by weighted $A$ may be highly noise, and the community extraction results based on weighted $A$ may be unstable. However, if the density of communities in $A$ is significant, but not comparable to the number of node pairs in the community, e.g. the number of edges in $C_k$ is in the order of $O(|C_k|)$.
% \end{enumerate}






%	\begin{equation}
%		\frac{S_{ik}}{|C_k|^\alpha} > \frac{S_{il}}{|C_l|^\alpha} \label{individual_update}
%	\end{equation}`
%The two sides in (\ref{individual_update}) can be viewed as rescaled measures of connectivity between the node $i$ and the two communities. When $\alpha=1$, both sides of Equation (\ref{individual_update}) have the interpretation of the averaged weights of parts between node $i$ and communities $C_k$ and $C_l$. Therefore, our method assigns each node $i$ to the community it is most tightly connected to.\\
%
%We now look at the impact of $\alpha$ on the eventual community detection outcome. Without loss of generality, we assume $|C_k|\geq |C_l|$. Rewriting (\ref{individual_update}) as:






% \subsection{Consistency of community detection under the Stochastic Blockmodel}
% 
% The formulation of (\ref{JCDC}), though not a direct extension of, matches the spirit of the Stochastic Blockmodel in the sense that they both regard the variance of edge densities in different parts of the network as mainly caused by the community assignments of the nodes involved. Therefore, we expect that our method produces asymptotically consistent community detection result under the block model. We state the consistency theorem below:\\
% 
% {\bf Theorem 1} Let all weights are the same, i.e., consider a binary network $A$. If for any community indices $a\neq b$, we have
% \begin{equation}
% \alpha(P_{aa}+P_{bb})>2P_{ab} \label{consistency}
% \end{equation}
% for $\alpha\geq 1$, or
% \begin{equation}
% (2^\alpha-1)\cdot\min(P_{aa}, P_{bb})>P_{ab}
% \end{equation}
% for $0<\alpha<1$, and the regularity conditions in \cite{Zhaoetal2012} are satisfied, then the JCDC (\ref{JCDC}) is strongly consistent when $\lambda_n/\log n\to+\infty$ and weakly consistent when $\lambda_n\to+\infty$ under the Stochastic Blockmodel as $n\to \infty$.\\
% 
% The proof is in the Appendix.\\
% 
% We clarify here that despite the fact that smaller $\alpha$ yields a stronger condition (\ref{consistency}), it does not mean a small $\alpha$ is worse than a large $\alpha$. First, currently there are no established theoretical results on convergence rates of any criterion under the Stochastic Blockmodel, or any other (more sophisticated) generative models. Second, the theorem states asymptotic properties, which may differ significantly for the networks with limited sizes.


%\subsection{The role of $w_{\max}$}\label{impact_of_wmax}

% the impact of the edge weights on the community detection results. Notice that both $\beta$ and $w_{\max}$ control the magnitude of the influence of features on the community detection results, therefore it is important to clarify the differences in their roles. In our method, the node features influence the detection results via edge weights. The parameters $\beta$ controls the influences of different features on the scalar edge weights $w_{ij}$'s, and $w_{\max}$ controls the impact of $w_{ij}$'s on the final detection results:
%\begin{center}
%\begin{minipage}[H, c]{0.4\textwidth} 
%\begin{tikzpicture}[->,>=stealth,shorten >=1pt, auto = center, node distance=3cm, 
%                    thick,data/.style={circle,draw,font=\sffamily\bfseries}, first para/.style={scale=0.7,draw,font=\sffamily\bfseries}, sec para/.style = {rectangle,scale=0.8, draw,dashed,font=\sffamily\Large\bfseries}] 
%\node[data] (fi) at (0, 4) {$\bm{f_i}$};
%\node[data] (fj) at (0, 2)  {$\bm{f_j}$};
%\node[data] (phiij) at (2, 3) {$\bm{\phi_{ij}}$};
%\node[data] (wij) at (4, 3) {$w_{ij}$};
%\node[data] (Aij) at (4, 1)  {$A_{ij}$};
%\node[data] (community) at (6, 2) {$C$};
%\node[data, draw=white] (beta) at (3,3.5) {$\beta$};
%\node[data, draw=white] (wmax) at (5.2,3) {$w_{\max}$};
%\foreach \from/\to in {fi/phiij, fj/phiij, phiij/wij, wij/community, Aij/community} 
%    \draw (\from) -> (\to); 
%\end{tikzpicture}  
%\end{minipage}
%\end{center}

%The tuning parameter $w_{\max}$ comes from our specific formulation of the function of $w$, however, its role in the joint community detection framework has a universal meaning shared by any methodology that addresses the same problem. The philosophical question is on balancing the influence of the network $A$ and the features $\bm{f_i}$'s. When both $A$ and $F$ display community structures that are not necessarily in agreement with each other, we need to decide how much influence each of them has on the final community detection result when combining the two sources of data. Such balance cannot be learned automatically from data, and in practice it is chosen in a subjective and context dependent fashion. In Section 6, we show a simulation that illustrates the varying impact of node features on the final detection result under different choices of $w_{\max}$.

%Specifically, we consider the scalar case in which we only have one feature and this features is correlated to the community structure of community $k$, i.e. $\mathbb{E}[\phi_{ij}|(i, j)\in e_k]>0$. The optimal $\beta$ has no closed form solution, thus we implement an approximation to illustrate this point for small $\beta$ values. The second order Taylor expansion of $w$ gives:
%\begin{align}
%w_{ij}& = w_{\max} - e^{\phi_{ij}\beta_k}\\
%&\approx w_{\max}-1+\phi_{ij}\beta_k - (\phi_{ij}\beta_k)^2/2 \label{taylor_order2}
%\end{align}
%The corresponding (approximated) term in JCDC is therefore $\sum_{(i, j)\ine_k}A_{ij}(2\phi_{ij}\beta_k - (\phi_{ij}\beta_k)^2)$ (ignoring the rescaling factor that does not affect $\hat{\beta}_k$), which gives
%\begin{align}
%\hat{\beta}_k &= \frac{\sum_{(i, j)\ine_k}\phi_{ij}}{\sum_{(i, j)\ine_k}\phi_{ij}^2} \to \frac{\mathbb{E}[\phi_{ij}|(i, j)\ine_k]}{Var[\phi_{ij}|(i, j)\ine_k] + \mathbb{E}[\phi_{ij}|(i, j)\ine_k]^2} \label{increasing function}
%\end{align}
%which shows that $\hat{\beta}_k$ is an increasing function of $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$ within a small neighborhood of 0, where the expansion (\ref{taylor_order2}) is a good approximation. As $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$ grows larger such monotonicity still holds but need to be shown in numerical evaluations.
%The approximation (\ref{taylor_order2}) is precise when $\phi_{ij}\beta_k$'s are small, and (\ref{increasing function}) shows that for small $\$We can see that in the neighbor hood $\hat{\beta}_k$ is positive and increase with $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$. When $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$ grows larger, the approximation (\ref{taylor_order2}) is not precise and we need to numerically evaluate to see the positive association between $\hat{\beta}_k$ and $\mathbb{E}[\phi_{ij}|(i, j)\ine_k]$.
%In practice, when the sample mean similarity within community $\hat{\mathbb{E}}[\phi_{ij}^{(z)}|(i, j)\in e_k]$ is large, the corresponding $\hat{\beta}^{(z)}$ is usually huge and dominating -- in the extreme case it is $\infty$ if all $\phi_{ij}^{(z)}$'s within the community have the same sign.


%The impact of $\beta$, however, is restricted to the stage in which the edge weights are determined. It mainly serves the purpose of balancing the influence of different features. We will see later that in our method, features that are more correlated to the estimated community structure tend to have a larger estimated $\beta$ coefficient. However, in practice, even the most correlated features may show significant differences in their clustering structure from that displayed in the network $A$, so the question of balancing the influences of $A$ and $F$ remains.\\

% \subsection{Interpretations of $\beta$}
% 
% With the formulation of $w(\cdot)$ chosen, it is natural to ask what the optimal $\beta$ means. Ideally, we expect to acquire a larger optimal $\beta^{(z)}$ if the corresponding $z$-th dimension $\phi^{(z)}$ is closely correlated with the community structure, i.e., there is a significant difference between the $\phi^{(z)}$ values within communities and between communities. This intuitive goal is the variable selection problem, an important practical aspect of all clustering methodology that makes use of multiple features or attribute information. Usually when people perform clustering techniques involving multiple features, it is of interest to know which dimensions in the features have essential connection to the clustering structure. The problem is relatively easier in supervised learning \cite{guoa2010modularized}, because the response in training data can be used to filter out irrelevant features. The problem is, however, much more difficult in unsupervised scenarios.\\
% 
% The joint community detection problem, for example, is a typical unsupervised learning problem. Specifically, in our approach the coefficient vector $\beta$, which carries the information of the significance of node features, is learnt along with the community structure. This creates difficulty in even defining the concept of significance of node features. Notice that it is relatively easy to define the conditional significance, which means that we fix a community structure, and define the significant node feature dimensions to be those that are significantly correlated with the estimated community structure. Clearly, such significance definition depends on the community structure. It is unclear though how to or whether it is meaningful to define a global significance. Recall that our final goal is to optimize the joint community detection criterion over $C$ and $\beta$ jointly, and currently the only feasible way is to optimize iteratively. Therefore, it is not unnatural that we base the feature selection and the related significance test on our best guess for the true underlying community structure, which is the estimated $C$.\\
% 
% In the discussion below, by "the community structure" we mean either the underground truth or a close guess. We aim at showing that our feature selection and testing methodology is effective in learning which dimensions are significantly correlated to the underlying community structure, if either we are in the oracle case and know the true community structure or have a close guess. One can view such feature selection and testing methodology as applied when the joint estimation is completed and mainly serves the interpretation of results. But the mechanism for this methodology - higher correlation with the estimated community structure yields larger estimated coefficient value - is consistent with our goal of joint community extraction. We optimize the joint community detection criterion iteratively, and throughout the procedure, we look for the possible agreement suggesting a certain community structure from both sources of information. Therefore, if a certain community assignment $C$ also separates certain dimension(s) of $\phi$, this suggests that we found the desired agreement on two types of evidence.\\
% 
% As an illustration of the methodology, let us consider a specific choice of $w_{ij}$ as in (\ref{weight_function}):
% \begin{equation}
% w(\bm{\phi_{ij}}, \beta):=w_{\max} - e^{-\langle \bm{\phi_{ij}}, \beta \rangle} \label{specific_choice}
% \end{equation}
% To study the location of the optimal $\beta$, we take the second order approximation to the exponential function, i.e.
% \begin{equation}
% 	w(t)\approx w_{\max}-1+t-\frac{t^2}{2} 
% \end{equation}
% where we write $w$ as a function of a scalar variable since in (\ref{specific_choice}) $w$ is determined by the inner product of its two vector arguments. Plugging the approximation of $w$ into  JCDC (\ref{JCDC}) and ignoring the constants that do no involve $\beta$, we have
% \begin{equation}
% 	R\approx\sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}\left( 2\beta'\bm{\phi_{ij}} -  \beta'(\bm{\phi_{ij}}\bm{\phi_{ij}}')\beta\right)
% \end{equation}
% Therefore the optimal $\beta$ is approximately:
% \begin{equation}
% 	\hat{\beta} = \left( \sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}(\bm{\phi_{ij}}\bm{\phi_{ij}}') \right)^{-1}\cdot \left( \sum_{k=1}^K\frac{1}{|C_k|^\alpha} \sum_{i, j\in C_k}A_{ij}\bm{\phi_{ij}} \right) \label{realized_version}
% \end{equation}
% 
% We simplify the problem by assuming that $A_{ij}$ is independent of $\bm{\phi_{ij}}$ given $C_k$, fixing the number of communities and assuming that as $n\to\infty$ the communities maintain the size ratios. We treat each $\bm{\phi_{ij}}$ as a realization of random variable $\phi$. For further simplicity, we assume the dimensions of $\phi$ to be identically distributed, having unit variance and equal covariance $\rho$ between each pair of different dimensions. We denote their common expectation by $u$. Therefore the population version($RHS_{pop}$) of the RHS in (\ref{realized_version}) is
% \begin{align}
% 	RHS_{pop} &= \left( (1-\rho)I + (\rho+u)\mathbbm{1}\mathbbm{1}' \right)^{-1}\cdot u\mathbbm{1}\\
% 			&= \frac{u Z}{1-\rho+(\rho+u) Z}\mathbbm{1}\label{illustration_beta}
% \end{align}
% where $Z$ is the dimension of $\phi$. It is then straightforward to see that the population version of the optimal $\hat{\beta}$, under the simplified case, is an increasing function of the total sum of $\mathbb{E}[\phi]$ in each of their corresponding dimensions. Switching back to the realization, this means that for the $z$-th feature, the more and larger positive $\phi_{ij}^{(z)}$ that we have within communities, the further $\hat{\bm{\theta}}^{(z)}$ departs from $0$ in the positive direction.\\


% \subsection{Penalty on $\beta$}




%{\bf Iterative optimization procedure:}
%\begin{enumerate}
%\item Initialize $\hat{C}$ and set $\bm{\hat{\beta}}=0$.
%\item Iterate until convergence
%	\begin{enumerate}
%	\item Fix $\bm{\hat{\beta}}$ and update $\hat{C}$
%		\begin{itemize}
%		\item Truncate negative edge weights to $0$.
%		\item Go through all nodes for multiple rounds. Within each round update each node's community assignment to the choice that maximizes JCDC
%		\end{itemize}
%	\item Fix $C$ and update $\bm{\hat{\beta}}$.
%	\end{enumerate}
%\item Perform the significance test on $\beta$ based on $\hat{C}$.
%\end{enumerate}




==> texsections/section_4_BACKUP.tex <==
 %\subsection{Comparison to benchmark methods}

We compare JCDC to three representative benchmark methods which use both the adjacency matrix and the node features: CASC (Covariate Assisted Spectral Clustering, \cite{binkiewicz2014covariate}), CESNA (Communities from Edge Structure and Node Attributes, \cite{yang2013community}), and BAGC (BAyesian Graph Clustering, \cite{xu2012model}).   In addition, we also include two standard methods that use either the network adjacency alone (SC, spectral clustering on the Laplacian regularized with a small constant $\tau = 1e-7$, as in \cite{Amini.et.al2013}), or the node features alone (KM, $K$-means performed on the $p$-dimensional node feature vectors, with 10 random initial starting values).   We generate networks with $n=150$ nodes and $K=2$ communities of sizes $100$ and $50$ from the degree-corrected stochastic block model as follows. The edges are generated independently with probability $\theta_i\theta_j p$ if nodes $i$ and $j$ are in the same community, and $r \theta_i\theta_j p$ if nodes $i$ and $j$ are in different communities.    We set $p=0.1$ and vary $r$ from $0.25$ to $0.75$.    We set $5\%$ of the nodes in each community to be ``hub'' nodes with the degree correction parameter $\theta_i=10$, and for the remaining nodes set $\theta_i=1$.   All resulting products are thresholded at 0.99 to ensure there are no probability values over 1.  These settings result in the average expected node degree ranging approximately from $22$ to $29$. 


\vspace{-2em}
\begin{figure*}[htbp]
	\centering
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/JCDC_results}
		\caption{JCDC,$w=5$}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/JCDC15_results}
		\caption{JCDC,$w=1.5$}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/SC_results}
		\caption{SC}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/KM_results}
		\caption{KM}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/CASC_results}
		\caption{CASC}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/CESNA_results}
		\caption{CESNA}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/BAGC_results}
		\caption{BAGC}
	\end{subfigure}
	\caption{Performance of different methods measured by normalized mutual information as a function of $r$ (out-in probability ratio) and $\mu$ (feature signal strength).}
	\label{fig_1}
\end{figure*}
\vspace{-2em}

% three bins with $5\%$ and $95\%$ quantiles of the corresponding node feature distribution, and then further partition the middle bin into smaller bins of length $0.5$.

For each node $i$, we generate $p = 2$ features, with one ``signal'' feature related to the community structure and one ``noise'' feature whose distribution is the same for all nodes.  The ``signal'' feature follows the distribution $N(\mu, 1)$ for nodes in community 1 and $N(-\mu, 1)$ for nodes in community 2, with $\mu$ varying from $0.5$ to $2$ (larger $\mu$ corresponds to stronger signal).  For use with CESNA, which only takes categorical node features, we discretize the continuous node features by partitioning the real line into 20 bins using $0.05, 0.1, \dots, 0.95$-th quantiles.  \tblue{For JCDC, based on the results in the Supplemental Material, we choose to use $\alpha=1$ and consider two possibilities of $w_n$, $w_n=1.5$ and $w_n=5$. Note that the larger $w_n$ is, the smaller the effect of the node features on community estimation.}    Finally, agreement between the estimated communities and the true community labels is measured by normalized mutual information, a measure commonly used in the network literature which ranges between 0 (random guessing) and 1 (perfect agreement). For each configuration, we repeat the experiments 30 times, and record the average NMI over 30 replications, shown as heatmaps in Figure \ref{fig_1}.


\tblue{Figure \ref{fig_1} compares the performance of our method, JCDC (a) and (b) to benchmark methods.   As expected, the performance of spectral clustering (c), which uses only the network information, is only affected by $r$ (the larger $r$ is, the more difficult the problem), and the performance of $K$-means (d), which uses only the features, is only affected by $\mu$ (the larger $\mu$ is, the easier the problem).   JCDC, however, is able to take advantage of both network and feature information, and its performance only deteriorates when neither is informative.  Figure \ref{fig_1} (e) to (g) show results for three benchmark methods that use both the network and the feature information.}   CASC (e)  appears to inherit the sharp phase transition from spectral clustering, which forms the basis of CASC, due perhaps to different community sizes and hub nodes, which are both challenging to spectral clustering;  CESNA (f) and BAGC (g) do not perform as well overall, with BAGC clustering all the hub nodes into one community most of the time.   


==> texsections/section_4__Yuan_Zhang____________2015-07-24_.tex <==
 %\subsection{Comparison to benchmark methods}

We compare JCDC to three representative benchmark methods which use both the adjacency matrix and the node features: CASC (Covariate Assisted Spectral Clustering, \cite{binkiewicz2014covariate}), CESNA (Communities from Edge Structure and Node Attributes, \cite{yang2013community}), and BAGC (BAyesian Graph Clustering, \cite{xu2012model}).   In addition, we also include two standard methods that use either the network adjacency alone (SC, spectral clustering on the Laplacian regularized with a small constant $\tau = 1e-7$, as in \cite{Amini.et.al2013}), or the node features alone (KM, $K$-means performed on the $p$-dimensional node feature vectors, with 10 random initial starting values).   We generate networks with $n=150$ nodes and $K=2$ communities of sizes $100$ and $50$ from the degree-corrected stochastic block model as follows. The edges are generated independently with probability $\theta_i\theta_j p$ if nodes $i$ and $j$ are in the same community, and $r \theta_i\theta_j p$ if nodes $i$ and $j$ are in different communities.    We set $p=0.1$ and vary $r$ from $0.25$ to $0.75$.    We set $5\%$ of the nodes in each community to be ``hub'' nodes with the degree correction parameter $\theta_i=10$, and for the remaining nodes set $\theta_i=1$.   All resulting products are thresholded at 0.99 to ensure there are no probability values over 1.  These settings result in the average expected node degree ranging approximately from $22$ to $29$. 


\vspace{-2em}
\begin{figure*}[htbp]
	\centering
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/JCDC_results}
		\caption{JCDC,$w=5$}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/JCDC15_results}
		\caption{JCDC,$w=1.5$}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/SC_results}
		\caption{SC}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/KM_results}
		\caption{KM}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/CASC_results}
		\caption{CASC}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/CESNA_results}
		\caption{CESNA}
	\end{subfigure}
	\begin{subfigure}[h]{0.135\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/BAGC_results}
		\caption{BAGC}
	\end{subfigure}
	\caption{Performance of different methods measured by normalized mutual information as a function of $r$ (out-in probability ratio) and $\mu$ (feature signal strength).}
	\label{fig_1}
\end{figure*}
\vspace{-2em}

% three bins with $5\%$ and $95\%$ quantiles of the corresponding node feature distribution, and then further partition the middle bin into smaller bins of length $0.5$.

For each node $i$, we generate $p = 2$ features, with one ``signal'' feature related to the community structure and one ``noise'' feature whose distribution is the same for all nodes.  The ``signal'' feature follows the distribution $N(\mu, 1)$ for nodes in community 1 and $N(-\mu, 1)$ for nodes in community 2, with $\mu$ varying from $0.5$ to $2$ (larger $\mu$ corresponds to stronger signal).  For use with CESNA, which only takes categorical node features, we discretize the continuous node features by partitioning the real line into 20 bins using $0.05, 0.1, \dots, 0.95$-th quantiles.  \tblue{For the JCDC, we use the tuning parameter values $\alpha=1$ and consider two choices of $w_n$, namely $w_n=1.5$ and $w_n=5$ throughout the paper,  based on our investigations of the tuning parameter impact reported in the Supplemental Material.  The smaller value of $w_n$ lets features to impact the community estimation, while the larger value of $w_n$ bases the estimation more on the network.}    Finally, agreement between the estimated communities and the true community labels is measured by normalized mutual information, a measure commonly used in the network literature which ranges between 0 (random guessing) and 1 (perfect agreement). For each configuration, we repeat the experiments 30 times, and record the average NMI over 30 replications, shown as heatmaps in Figure \ref{fig_1}.


\tblue{Figure \ref{fig_1} compares the performance of our method, JCDC (a) and (b) to benchmark methods.   As one would expect, the performance of spectral clustering (c), which uses only the network information, is only affected by $r$ (the larger $r$ is, the harder the problem), and the performance of $K$-means (d), which uses only the features, is only affected by $\mu$ (the larger $\mu$ is, the easier the problem).   JCDC, however, is able to take advantage of both network and feature information, and its performance only deteriorates when neither is informative.  The comparison between (a) and (b) suggests that when the clustering structure in the feature is not very clear and well-aligned with the community structure, giving features high impact on edge weights may be misleading for networks without a very clear community structure either, and it seems that doing so is only beneficial when features provide correct and much clearer community structure than the network.  Figure \ref{fig_1} (e) to (g) show results for three benchmark methods that all use both the network and the feature information.}   CASC (e)  appears to inherit the sharp phase transition from spectral clustering, which forms the basis of CASC, due perhaps to different community sizes and hub nodes, which are both challenging to spectral clustering;  CESNA (f) and BAGC (g) do not perform as well overall, with BAGC clustering all the hub nodes into one community most of the time.   


==> texsections/section_55.tex <==


\subsection{The Mexican political elite network}

%%%%%%%%%%%%%
%%%%%%%%%%%%% URL: https://sites.google.com/site/ucinetsoftware/datasets/mexicanpoliticalelite
%%%%%%%%%%%%%

The Mexican political elite network \cite{gil1996political,
  de2005exploratory} consists of 35 Mexican politicians including
presidents and their close associates. The edge between two
politicians indicates a significant tie of any type between them
(political, business, friendship, etc.).  There is one available
continuous node
feature, the year in which the person first assumed significant power
in the government.  We also know the politicians background --
military or civilian -- 
which we can compare to
detected communities.   In early years of the time period under
consideration, the military dominated the government, and over the
years civilian politicians gradually took over. The 
background partition and the community detection results by different
methods -- by our method (JCDC), modularity on the network alone, and
$K$-means on the year -- are shown in Figure \ref{mexican}.
\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=1]{fig/mexican.pdf}
\caption{Political background}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=3]{fig/mexican.pdf}
\caption{JCDC}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=2]{fig/mexican.pdf}
\caption{Modularity}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=4]{fig/mexican.pdf}
\caption{K-means}
\end{subfigure}
%\caption{Upper Left: Background; Upper Right: Modularity; Lower left: Our method; Lower Right: K-means}
\caption{The background partition (red: military, blue:civilian) and community detection results by different methods.}\label{mexican}
\end{figure}

The absorption of civilian politicians into the government was a
gradual process and there is no single cut-off threshold on year that
separates the backgrounds of politicians well. This explains why
$K$-means does not agree well with political background. On the other
hand, politicians stepping into power in years close to each other
tend to have similar backgrounds, which is accounted for by higher
edge weights in our method.  As measured by normalized mutual
information (NMI) between estimated communities and the background partition, our method (NMI=0.37) outperforms both modularity
(NMI=0.20) and $K$-means (NMI=0.26).   The same holds for the Jaccard
Index(JI): our method achieves JI=0.85, modularity JI=0.74, and
$K$-means JI=0.66. The estimated $\bm{\beta}$ is $(1.59, 1.04)$ with
permutation test based $p$-values of $(0.02, 0.00)$.  This indicates
that our method recognizes the year as a significant feature in
formation of both estimated communities.

\subsection{The Lawyer friendship network}

%%%%%%%%%%%%%
%%%%%%%%%%%%% URL: http://www.stats.ox.ac.uk/~snijders/siena/Lazega_lawyers_data.htm
%%%%%%%%%%%%%


The Lawyer friendship network \cite{lazega2001collegial} consists of
71 lawyers in a Northeastern US corporate law
firm. The edges indicate friendship ties between lawyers. There are 7
features available on each node: status (partner or associate),
gender, office location (Boston or Hartford), years with the firm,
age, practice (litigation or corporate) and law school attended
(Harvard, Yale, University of Connecticut, or other). We eliminated 6
isolated nodes with zero degrees.  Figure \ref{adj_lawyers} shows heat
plots of the adjacency matrix rearranged by sorting the columns and
the rows of the original adjacency matrix in ascending order by each
feature.  Partition by office location (Figure \ref{adj_lawyers}(c))
shows the clearest community structure, and thus we will use partition
by office
location to compare to community detection on the network
using all the other variables as node features.    In this comparison,
we omit the very small Providence office, which has only two non-isolated nodes and only two edges to other nodes.
\begin{figure}[h]
 \centering
 \begin{subfigure}[b]{0.13\textwidth}
  \includegraphics[width=\textwidth, page=1]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A2.jpeg}
  \caption{status}
 \end{subfigure}
 \begin{subfigure}[b]{0.13\textwidth}
   \includegraphics[width=\textwidth, page=2]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A3.jpeg}
  \caption{gender}
 \end{subfigure}
 \begin{subfigure}[b]{0.13\textwidth}
   \includegraphics[width=\textwidth, page=3]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A4.jpeg}
  \caption{office}
 \end{subfigure}
 \begin{subfigure}[b]{0.13\textwidth}
   \includegraphics[width=\textwidth, page=4]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A5.jpeg}
  \caption{year}
 \end{subfigure}
 \begin{subfigure}[b]{0.13\textwidth}
   \includegraphics[width=\textwidth, page=5]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A6.jpeg}
  \caption{age}
 \end{subfigure}
 \begin{subfigure}[b]{0.13\textwidth}
   \includegraphics[width=\textwidth, page=6]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A7.jpeg}
  \caption{practice}
 \end{subfigure}
 \begin{subfigure}[b]{0.13\textwidth}
   \includegraphics[width=\textwidth, page=7]{fig/lawyers_grouping.pdf}
%   \includegraphics[width=\textwidth, page=1]{fig/Lawyer_A/A8.jpeg}
  \caption{school}
 \end{subfigure}
 \caption{Adjacency matrices aligned along each marginal feature}\label{adj_lawyers}
\end{figure}


The estimated community structures by different methods and the true office location partition are shown in Figure \ref{lawyers}. Our method achives a mutual information of 0.34 to the true office partition, while modularity and K-means achive 0.02 and 0.00 respectively. Measuring the results in Jaccard Index, our method achieves a precision of 0.85 while modularity and K-means achive 0.56 and 0.54 respectively.
\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=1]{fig/lawyers.pdf}
\caption{Political background}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=3]{fig/lawyers.pdf}
\caption{JCDC}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=2]{fig/lawyers.pdf}
\caption{Modularity}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth, page=4]{fig/lawyers.pdf}
\caption{K-means}
\end{subfigure}
%\caption{Upper Left: Background; Upper Right: Modularity; Lower left: Our method; Lower Right: K-means}
\caption{The office location partition and community detection results from different methods}\label{lawyers}
\end{figure}

The estimated $\bm{\beta}$ by our method is:
\begin{table}[H]
 \caption{Estimated $\bm{\beta}$ and their p-values}
 \begin{center}
  \begin{tabular}{|c|c|c|c|c|c|c|}\hline
	        & status & gender & year & age & practice & school\\\hline
   Community 1  & 0.38(0.00)  &   0.02(0.31)  & 0.15(0.12) & 0.18(0.10) &   0.15(0.048)  & 0.00(0.37)\\\hline
   Community 2  & 0.05(0.10)  &   0.00(0.32)  & 0.07(0.12) & 0.03(0.17) &   0.00(0.31)  & 0.00(0.28)\\\hline
  \end{tabular}
 \end{center}
\end{table}
Our method identifies status and practice as the features that relate to the first community and recognized no specific feature that significantly relates to the second community. This suggests that node features assist our method in extracting the first community, while our method extracts the second community based mainly on information from the network.

% \begin{table}[H]
%  \caption{Community detection precisions}
%  \begin{center}
%   \begin{tabular}{|c|c|c|c|}\hline
% 	               & Our method & N-G Modularity & K-means\\\hline
%    Mutual Information  &    0.34    &     0.02       &  0.00 \\\hline
%    Jaccard Index       &    0.85    &     0.56       &  0.54 \\\hline
%   \end{tabular}
%  \end{center}
% \end{table}

==> texsections/section_5__Yuan_Zhang____________2015-07-24_.tex <==
\subsection{The world trade network}

%%%
%%% URL: http://vlado.fmf.uni-lj.si/pub/networks/data/esna/metalWT.htm
%%%

The world trade network \cite{de2011Pajek} connects 80 countries based on the amount of trade of metal manufactures between them, in the year 1994 or when not available for that year,  in 1993 or 1995.   Nodes are countries and edges represent positive amount of import and/or export between the countries.  Each country also has three categorical features: the continent  (Africa, Asia, Europe, North America, South America, and Oceania), the country's structural position in the world system in 1980 (core, strong semi-periphery, weak semi-periphery, periphery) and in 1994 (core, semi-periphery, periphery). Figures \ref{worldtrade} (a) to (c) show the adjacency matrix rearranged by sorting the nodes by each of the features.  Partition into continents (Figure \ref{worldtrade}(a)) clearly shows community structure, whereas the other two features show hubs (core status countries trade with everyone), and no assortative community structure.   We will thus compare partitions found by all the competing methods to the continents, and omit the three Oceania countries from further analysis because no method is likely to detect such a small community.    The two world position variables ('80 and '94) will be used as features, treated as ordinal variables. % The tuning parameters for JCDC are again set to $w_n=1.5$ and $\alpha=1$, and All settings for all methods are the same as those used for simulated data.

\setcounter{subfigure}{0}
\begin{figure*}[b]
	\centering
	\begin{subfigure}[b]{0.19\textwidth}
	\includegraphics[width=\textwidth]{fig/A_continent.pdf}
	\caption{A by continent}
	\end{subfigure}
	\begin{subfigure}[b]{0.19\textwidth}
	\includegraphics[width=\textwidth]{fig/A_world_system_1980.pdf}
	\caption{A by position '80}
	\end{subfigure}
	\begin{subfigure}[b]{0.19\textwidth}
	\includegraphics[width=\textwidth]{fig/A_world_system.pdf}
	\caption{A by position '94}
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_true.pdf}
		\caption{Continent\\\ }
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_JCDC.pdf}
		\caption{JCDC,$w=5$\\NMI=0.54}
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
			\includegraphics[width=\textwidth]{fig/WorldTrade_JCDC15.pdf}
			\caption{JCDC,$w=1.5$\\NMI=0.50}
		\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_SC.pdf}
		\caption{SC\\NMI=0.47}
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_KM.pdf}
		\caption{KM\\NMI=0.25}
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_CASC.pdf}
		\caption{CASC\\NMI=0.39}
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_CESNA.pdf}
		\caption{CESNA\\NMI=0.26}
	\end{subfigure}
	\begin{subfigure}[b]{0.16\textwidth}
		\includegraphics[width=\textwidth]{fig/WorldTrade_BAGC.pdf}
		\caption{BAGC\\NMI=0.11}
	\end{subfigure}

	\caption{(a)-(c): the adjacency matrix ordered by different node features; (d) network with nodes colored by continent (taken as ground truth); blue is Africa, red is Asia, green is Europe, cyan is N.\ America and purple is S.\ America.  (e)-(k) community detection results from different methods;  colors are matched to (d) in the best way possible. }\label{worldtrade}
\end{figure*}



%\tblue{Measured by the normalized mutual information(NMI), JCDC, CASC, CESNA, BAGC, SC and K-means achieve 0.536, 0.450, 0.257, 0.109, 0.467 and 0.226 respectively. 
The results for all methods are shown in Figure \ref{worldtrade}, along with NMI values comparing the detected partition to the continents.  All methods were run with the true value $K=5$.
%, but both JCDC and BAGC returned some communities empty.   The community missed by JCDC is Africa (shown in blue in Figure \ref{worldtrade} (d) and also as the small block in the bottom-left corner of Figure \ref{worldtrade} (a)), which has more edges to other communities than within itself.   Since JCDC is only designed to detect assortative community structure, it merges these nodes into other communities to which they have more connections. 

% % %The difference between JCDC and CASC, especially on Europe (green) which contains 35\% of all nodes, is likely due to CASC favoring more balanced community sizes, a feature it inherits from spectral clustering.  CASC here performs similarly to spectral clustering, whereas CESNA and BAGC both fail to recover the continent partition. 
\tblue{Figure \ref{worldtrade} (e) shows that JCDC favoring the network estimates communities N. America, S. America and Asia with high accuracy and roughly splits community Europe arbitrarily into two communities, possibly due to that the specified community number is in force. Notice that no method can successfully estimate community Africa -- not even close, likely a result of its disassortative nature, telling from (a).}



%We also conducted the permutation test in JCDC to determine whether the two available features are relevant to community structure.   The empirical significance test suggests that the world position in 1994 is significantly correlated (at significance level of 0.05) with three out of four communities found by JCDC, whereas world position in 1980 is not significant in any of the communities.   This makes sense considering that the trade data from which the network is constructed covers the period 1993-1995.   

%\vspace{-2em}
%\begin{table}[h]
%\caption{Feature coefficients $\hat{\beta}_k$ estimated by JCDC and their $p$-values. Best match is determined by majority vote.}
% \begin{tabular}{llll}
%Community	& Best match	& Position '80 & Position '94\\\hline
%blue	& Europe 	& {\bf 0.006(0.00)}	& 0.198(1.00)\\
%red  	& Asia		& {\bf 0.189(0.00)}	& 0.000(1.00)\\
%green	& Europe 	& 0.331(1.00)	& {\bf 0.109(0.00)}\\
%cyan 	& N. America & 0.088(1.00) & 0.000(1.00)\\
%purple & S. America & 0.000(1.00)	& 0.000(1.00)\\\hline
%\end{tabular}
%\label{table:worldtrade}
%\end{table}


\vspace{-2em}
\begin{table}[h]
\caption{Feature coefficients $\hat{\beta}_k$ estimated by JCDC. Best match is determined by majority vote.}
 \begin{tabular}{llll}
Community	& Best match	& Position '80 & Position '94\\\hline
blue	& Europe 	& 0.000	& 0.143\\
red  	& Asia		& 0.314	& 0.127\\
green	& Europe 	& 0.017	& 0.204\\
cyan 	& N. America & 0.107 & 0.000\\
purple & S. America & 0.121	& 0.000\\\hline
\end{tabular}
\label{table:worldtrade}
\end{table}




\subsection{The lawyer friendship network}

%%%
%%% URL: http://www.stats.ox.ac.uk/~snijders/siena/Lazega_lawyers_data.htm
%%%

The second dataset we consider is the lawyer friendship network \cite{lazega2001collegial}, which consists of 71 lawyers in a Northeastern American corporate law firm. The edges indicate friendships between the lawyers. There are seven features available for each node: status (partner or associate), gender, office location (Boston, Hartford, or Providence, a very small office with only two non-isolated nodes), years with the firm, age, practice (litigation or corporate) and law school attended (Harvard, Yale, University of Connecticut, or other).  Categorical features with $M$ levels are represented by $M-1$ dummy indicator variables.  We eliminated six isolated nodes with zero degrees.  Figures \ref{lawyers} (a)-(g) show heatmap plots of the adjacency matrix with nodes sorted by each feature.  Partition by status (Figure \ref{lawyers}(a)) shows the strongest community structure, and thus we will compare community detection results to the status partition.   
%    In this comparison, we omit the very small office, which has only two non-isolated nodes and only two edges to other nodes.
\setcounter{subfigure}{0}
\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth]{fig/A_status.pdf} 
	\caption{$A$ by status}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth]{fig/A_gender.pdf}
	\caption{$A$ by gender}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth]{fig/A_office.pdf} 
	\caption{$A$ by office}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth, page=4]{fig/lawyers_grouping.pdf}
	\caption{$A$ by years}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth, page=5]{fig/lawyers_grouping.pdf} 
	\caption{$A$ by age}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth]{fig/A_practice.pdf} 
	\caption{$A$ by practice}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
	\includegraphics[width=\textwidth]{fig/A_school.pdf} 
	\caption{$A$ by school}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_true.pdf}
		\caption{Status\\\ }
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_JCDC.pdf}
		\caption{JCDC,$w=5$\\NMI=0.54}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_JCDC15.pdf}
		\caption{JCDC,$w=1.5$\\NMI=0.50}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_SC.pdf}
		\caption{SC\\NMI=0.44}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_KM.pdf}
		\caption{KM\\NMI=0.44}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_CASC.pdf}
		\caption{CASC\\NMI=0.49}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_CESNA.pdf}
		\caption{CESNA\\NMI=0.07}
	\end{subfigure}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{fig/Lawyers_BAGC.pdf}
		\caption{BAGC\\NMI=0.20}
	\end{subfigure}

	\caption{(a)-(g): adjacency matrix with nodes sorted by features; (h): network with nodes colored by status (blue is partner, red is associate); (i)-(n): community detection results from different methods. }\label{lawyers}
\end{figure*}

% \tblue{  Comparing the estimated communities to the status partition, JCDC, CASC, CENSA, BAGC, SC and KM achieve normalized mutual information of 0.721, 0.480, 0.084, 0.197, 0.496 and 0.416 respectively. }

Communities estimated by different methods are shown in Figure \ref{lawyers} (i)-(o), all run with $K = 2$. 
%    For JCDC, all estimated feature coefficients are not significant, which suggests the community structure in the adjacency matrix is strong enough to be recovered without using the features, even though the features do contain some information about the communities as suggested by the result of $K$-means.  
\tblue{Compared to the partition of status, JCDC estimates assign a few nodes in community associate that have rivally many  within- and between-community edges to the other community; while CASC produces unbalanced estimated communities in the opposite way -- this is likely due to the impact from features.}  Spectral clustering performs somewhat worse, perhaps due to the presence of hub nodes.    CASC does improve upon both spectral clustering and $K$-means by using the feature information, but its NMI is not as high as that of JCDC.   CESNA and BAGC do not perform well (though here BAGC does better than CESNA, whereas in the first example it was the other way around), possibly because of weak feature signals or hub nodes, or because they detect community structure corresponding to something other than status.  


\begin{table}[h]
\caption{Feature coefficients $\hat{\beta}_k$ estimated by JCDC and their $p$-values.}
 \begin{tabular}{lllllll}
Comm.	& gender	& office& years	& age		& practice		& school\\\hline
blue		& 0.290 & 0.532 & 0.212	& 0.390 & 0.095 & 0.000\\	
red			& 0.012 & 0.378 & 0.725	& 0.320 & 0.118 & 0.097\\\hline
\end{tabular}
\label{table:worldtrade}
\end{table}

%\begin{table}[h]
%\caption{Feature coefficients $\hat{\beta}_k$ estimated by JCDC and their $p$-values.}
% \begin{tabular}{llll}
%Comm.	& gender	& office& years\\\hline
%blue		& 0.290 & 0.532 & 0.212\\	
%red			& 0.012 & 0.378 & 0.725\\\hline
%			& age		& practice		& school\\\hline
%blue		& 0.390 & 0.095 & 0.000\\
%red			& 0.320 & 0.118 & 0.097\\\hline
%\end{tabular}
%\label{table:worldtrade}
%\end{table}



%
%\begin{table}[h]
%\caption{Feature coefficients $\hat{\beta}_k$ estimated by JCDC and their $p$-values.}
% \begin{tabular}{lllll}
%Comm.	& gender	& office-Bos.	& office-Hart.	& years\\\hline
%blue		& 0.280(1.00) & 0.466(1.00) & 0.171(1.00) & 0.304(1.00)\\	
%red			& 0.000(1.00) & 0.396(1.00) & 0.168(1.00) & 0.588(1.00)\\\hline
%			& age		& practice		& school-H./Y.	& school-UCon\\\hline
%blue		& 0.432(1.00) & 0.069(1.00) & 0.000(1.00) & {\bf 0.040(0.000)}\\
%red			& 0.366(1.00) & {\bf 0.113(0.00)} & 0.356(1.00) & 0.000(1.00)\\\hline
%\end{tabular}
%\label{table:worldtrade}
%\end{table}




==> texsections/section_6__Yuan_Zhang____________2015-07-24_.tex <==
Our method incorporates feature-based weights into a community detection criterion which allows it to potentially improve detection compared to using just the adjacency matrix or just clustering the node features.   It has the ability to estimate coefficients for each feature within each community and thus learn which features are correlated with the community structure and which are not, which is key to good performance in realistic scenarios.   The community detection criterion we use is designed for assortative community structure, with more connections within communities than between, and benefits the most from using features that have a similar clustering structure.   

There are several directions in which this method can be improved or extended.   Variation in node degrees, often modeled via the degree-corrected stochastic block model \cite{Karrer10} which regards degrees as independent of community structure, may in some cases be correlated with node features, and accounting for degree variation jointly with features can potentially further improve detection.  Another useful extension is to overlapping communities.  One possible way to do that is to optimize each summand in JCDC \eqref{JCDC} separately and in parallel, which can create overlaps, but would require careful initialization in order to avoid all communities converging to the same set of nodes.  Statistical models that specify exactly how features are related to community assignments and edge probabilities can also be useful, though empirically we found no such standard models that could compete with the non-model-based JCDC on real data.   This suggests that more involved and perhaps data-specific modeling will be necessary to accurately describe real networks, and some of the techniques used here, such as community-specific feature coefficients and model selection by permutation tests, could be useful in that context as well.  



==> texsections/tuning__Yuan_Zhang____________2015-07-24_.tex <==
%\subsection{The impact of tuning parameters}
\label{sec:tuning}

The JCDC method uses two user-selected tuning parameters, $\alpha$ and $w_n$.  Here we conduct numerical experiments on the impact of tuning parameters.  The tuning parameters suggested by these experiments are fixed throughout the manuscript for both simulated and real networks.

First we evaluate the impact of $\alpha$, which determines the algorithm's preference for larger or smaller communities.  Thus we study its effect on the estimated community size as well as detection accuracy.  For this experiment, we generate data from a stochastic block model with $n=120$ nodes and $K=2$ communities. We set the within-community edge probabilities to  $0.3$ and between-community edge probabilities to be $0.15$, and vary $n_1$, the number of nodes in the larger community, from 60 to 100.   Since $\alpha$ is a tuning parameter of the community detection criterion and is not related to feature weights, we set features to a constant, resulting in unweighted networks.   The results are averaged over 50 replications.  

%\vspace{-3em}
\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth, page=1]{fig/alpha.pdf}
\caption{The size of the larger estimated community}
\label{fig_2a}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth, page=2]{fig/alpha.pdf}
\caption{Community detection accuracy} 
\label{fig_2b}
\end{subfigure}
\caption{Results for varying tuning parameter $\alpha$. Solid lines correspond to JCDC, horizontal dotted lines to spectral clustering, which does not depend on $\alpha$.}
\label{fig_2}
\end{figure}


 Since $\alpha$ affects community sizes, we report the size of the larger estimated community (Figure \ref{fig_2}(a)) as well as the accuracy of community detection as measured by normalized mutual information. For comparison, we also record the results from spectral clustering (horizontal lines in Figure \ref{fig_2}), which do not depend on $\alpha$.   When communities are balanced ($n_1 = n_2 = 60$),  JCDC performs well for all values of $\alpha$, producing balanced communities and uniformly outperforming spectral clustering.   The larger values of $\alpha$ in JCDC result in more balanced communities, while the smaller $\alpha$'s tend to produce a large and a small community;   spectral clustering, on the other hands, is biased towards balanced communities.    In terms of community detection accuracy, Figure \ref{fig_2} (b) shows that the JCDC method outperforms spectral clustering over a fairly wide range of values of $\alpha$, and this range depends on how unbalanced the communities are.  For simplicity and ease of interpretation of the criterion, we set $\alpha = 1$ for all the simulations and data analysis reported in the main manuscript;  however, it can be changed by the user if a priori information about community sizes is available.  

%\vspace{-2em}

Next, we investigate the impact of $w_n$, which controls the influence of features.  To investigate the trade-off between the two sources of information (network and features),  we generate two different community partitions.  Specifically, we consider two communities of sizes $n_1$ and $n_2$, $n_1 + n_2 = n = 120$. We generate two label vectors $c^A$ and $c^F$, with $c^A_i=1$ for $i=1,\ldots, n_1$ and $c^A_i=2$ for $i=n_1+1,\ldots, n$, while the other vector has $c^F_i=1$ for $i=1,\ldots, n_2$ and $c^F_i=2$ for $i=n_2+1, \ldots, n$.  Then the edges are generated based on $c^A$ with the node features generated based on $c^F$.  We generate 2 node features: feature 1 follows $N(\mu, 1)$ for node $i$ if $c_i^F=1$ and $N(0, 1)$ if $c_i^F=2$; feature 2 follows $N(0, 1)$ if $c_i^F=1$ and $N(-\mu, 1)$ if $c_i^F=2$. We fix $\mu=3$ and set $\alpha=1$. We set the within- and between-community edge probabilities the same as the previous simulation and vary the values of $w_n$ from $1.1$ to $2$ and inspect the agreement between the estimated communities $\hat{e}$ and $c_A$ and $c_F$, respectively.  Since the $n_1=n_2=60$ case yields $c^A=c^F$, we change the range of $n_1$ to $[70, 110]$ in this simulation.  The results are shown in Figure \ref{fig_3}.

%\vspace{-3em}
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{fig/w}%%%%%%%%
\caption{Impact of $w_n$ on the resemblance of the estimated community structure $\hat{e}$ to the community structures in the network $c_A$ and in node features $c_F$, in presence of a discrepancy between them. Solid lines correspond to normalized mutual information between $\hat{e}$ and $c_A$, and dotted lines correspond to normalized mutual information between $\hat{e}$ and $c_F$. Lines numbered 1, $\ldots$, 5 correspond to larger community sizes of 70, $\ldots$, 110 respectively.}
\label{fig_3}
\end{figure}
%\vspace{-2em}

As we can see, in general, when $w_n$ is small and $r$ is not very large, the estimated community structure agrees more with $c^F$ than with $c^A$.  When $w_n$ increases, the estimated $\hat{e}$ becomes more similar to $c^A$. This again agrees with the discussion in previous sections, i.e., the first term in \eqref{break_JCDC_to_two_terms} dominates the second one when $w_n$ is large enough.  Further, as $r$ increases, the community structure in the network becomes more prominent, thus $\hat{e}$ becomes more similar to $c^A$.  It is also interesting to note that the rate at which the similarity between $\hat{e}$ and $c^F$ decreases is lower than that at which the similarity between $\hat{e}$ and $c^A$ increases.  This suggests that in practice, one may consider to use a relatively large value of $w_n$.

